Impact of string interactions on the space-time evolution of hadronic vertices

We investigate the space-time picture of string evolution and hadron production in a fully string-based model for high energy collisions involving heavy ions. We find that although the density strings is quite large at the time of hadronization in a central heavy ion collision, the initial overlap between them right after the collisions is not necessarily large. We also find that when including string--string interactions using the so-called shoving model, the density of strings is decreased which should dampen the rapid increase in string tension in the rope hadronization with multiplicity that we found in a previous paper.

==> figs/PbPb-1.tex <==
\ECirc(-9.13541,-7.90953){0.353312}
\ECirc(24.2252,30.9077){0.612132}
\ECirc(22.0819,-40.1359){1.33308}
\ECirc(18.1423,-39.6021){0.685048}
\ECirc(46.4385,-12.4939){0.903072}
\ECirc(22.4475,-26.851){0.880264}
\ECirc(-21.3047,-7.75417){0.584636}
\ECirc(27.9475,35.5734){1.55521}
\ECirc(-1.38492,47.8451){1.20741}
\ECirc(5.27468,-51.2733){1.46057}
\ECirc(4.08135,-49.0907){1.55946}
\ECirc(18.6189,-21.4109){0.792156}
\ECirc(-21.6177,-22.9013){0.96173}
\ECirc(-23.7902,-41.4539){0.960489}
\ECirc(-59.263,16.3552){1.31975}
\ECirc(0.121228,-67.8165){0.676442}
\ECirc(35.5623,49.7803){0.649324}
\ECirc(-33.208,5.30184){0.616139}
\ECirc(-24.4613,-7.48646){0.603563}
\ECirc(-26.9512,23.0903){0.370743}
\ECirc(6.24122,-21.6692){0.594189}
\ECirc(10.7291,-4.17182){0.663995}
\ECirc(-13.7728,-25.6724){0.494959}
\ECirc(-9.9601,48.102){0.69365}
\ECirc(4.92074,35.2964){0.943493}
\ECirc(6.57776,38.4789){0.925337}
\ECirc(12.4595,-48.7985){0.307595}
\ECirc(-33.237,-14.315){0.665117}
\ECirc(25.4546,40.0483){0.577591}
\ECirc(24.0266,34.7038){0.680897}
\ECirc(-36.3778,13.3934){0.604691}
\ECirc(-24.4426,5.35331){0.653516}
\ECirc(28.1614,37.2128){0.367159}
\ECirc(-37.6141,-40.7656){0.700551}
\ECirc(38.9123,-0.32523){0.499891}
\ECirc(-23.3835,45.5334){0.836783}
\ECirc(5.62734,-52.162){0.930878}
\ECirc(-38.2029,-3.16135){0.414308}
\ECirc(24.6988,-15.0983){0.594827}
\ECirc(21.9725,-38.9601){0.461908}
\ECirc(5.51095,-49.541){0.577818}
\ECirc(4.77905,-48.906){1.14425}
\ECirc(-37.4088,-7.73738){0.883017}
\ECirc(-38.228,-34.6548){1.25586}
\ECirc(13.3494,-48.1809){0.819623}
\ECirc(23.205,30.2122){0.534253}
\ECirc(6.64464,55.8642){1.17036}
\ECirc(-7.17536,46.5104){0.601616}
\ECirc(-5.19374,43.6933){0.416227}
\ECirc(-2.38695,43.7227){0.459981}
\ECirc(-21.9978,-9.83193){0.671001}
\ECirc(11.0489,-48.4055){0.590428}
\ECirc(9.43325,-52.8183){0.342519}
\ECirc(4.55193,-13.8576){0.699687}
\ECirc(27.8971,8.58396){1.11027}
\ECirc(-38.998,14.5912){0.447031}
\ECirc(-4.25594,-20.2897){0.651962}
\ECirc(20.406,-11.1852){0.655028}
\ECirc(-40.2439,31.3384){0.659061}
\ECirc(42.0361,-8.77052){0.404743}
\ECirc(50.8133,-24.8111){0.816769}
\ECirc(-1.66175,0.975552){1.39776}
\ECirc(7.33035,-52.6857){0.454391}
\ECirc(5.56625,40.333){0.669982}
\ECirc(6.03033,39.0072){0.572047}
\ECirc(-4.80871,-7.65149){1.83876}
\ECirc(-22.6545,-19.8136){0.445716}
\ECirc(-8.41035,-36.9507){0.954999}
\ECirc(-52.4979,8.62764){0.52064}
\ECirc(-0.585052,-22.595){0.857921}
\ECirc(20.7518,30.5687){1.47557}
\ECirc(-36.674,42.7071){0.42076}
\ECirc(-37.2302,37.8442){0.514133}
\ECirc(19.5107,-39.1533){1.01175}
\ECirc(38.2414,33.457){1.33366}
\ECirc(7.27954,-9.38351){0.340638}
\ECirc(-32.1354,-5.24218){1.32018}
\ECirc(-13.2573,6.20151){0.551148}
\ECirc(28.3409,36.0295){0.704107}
\ECirc(11.7505,-13.9176){0.776262}
\ECirc(14.2182,-12.1634){0.446822}
\ECirc(-11.6986,-36.8189){0.336032}
\ECirc(-10.231,-3.54274){0.796158}
\ECirc(12.5492,5.65374){0.601153}
\ECirc(-35.9243,13.9473){0.590671}
\ECirc(-35.5422,17.1143){0.541576}
\ECirc(-30.0181,3.76914){0.453323}
\ECirc(-15.8753,-40.3023){1.9473}
\ECirc(-15.7494,-28.2572){0.765423}
\ECirc(19.3566,-38.7133){0.597633}
\ECirc(42.3186,7.59332){0.702101}
\ECirc(17.2932,-2.01094){0.725938}
\ECirc(-20.1206,-10.271){0.674809}
\ECirc(20.6629,5.59298){0.609276}
\ECirc(-43.3045,-4.7429){0.692324}
\ECirc(30.6799,19.4392){0.690106}
\ECirc(-52.4016,-27.9126){0.691579}
\ECirc(-39.8279,-8.30995){0.78843}
\ECirc(-21.9351,-6.97531){0.269672}
\ECirc(10.247,-50.0441){0.568198}
\ECirc(-22.4615,-22.9406){2.14656}
\ECirc(-1.3111,51.7318){0.653749}
\ECirc(-12.2165,-57.0396){1.65481}
\ECirc(28.2892,-9.47578){0.692025}
\ECirc(55.8369,-3.19347){1.57991}
\ECirc(55.8809,-4.287){0.782242}
\ECirc(57.0376,-2.6392){0.50115}
\ECirc(-7.70552,6.98667){0.633938}
\ECirc(20.2835,-35.9108){1.45258}
\ECirc(-3.67423,49.7389){0.903706}
\ECirc(7.79046,-31.208){0.698043}
\ECirc(-61.985,8.51745){0.63238}
\ECirc(-13.3725,49.073){1.08025}
\ECirc(-13.8514,48.6969){1.08025}
\ECirc(-14.7113,-23.9423){0.704474}
\ECirc(21.2506,-23.1195){0.915691}
\ECirc(-24.1462,-7.11621){1.0766}
\ECirc(44.648,-32.3504){0.825892}
\ECirc(-10.5027,-6.71152){0.732551}
\ECirc(8.11698,35.4793){0.693247}
\ECirc(8.38912,36.2144){0.427814}
\ECirc(64.762,-16.7287){0.65796}
\ECirc(-7.47904,15.2033){1.28121}
\ECirc(-1.48556,16.7509){0.854577}
\ECirc(-26.7736,42.9393){3.40819}
\ECirc(-24.3864,37.6461){0.465364}
\ECirc(-3.25297,12.9483){0.743069}
\ECirc(-2.42129,12.2117){0.290778}
\ECirc(3.16776,8.86843){0.287154}
\ECirc(-39.699,-8.93973){0.251312}
\ECirc(-57.5529,40.4935){1.29035}
\ECirc(23.9516,29.4688){0.573727}
\ECirc(3.22485,-2.57594){0.490825}
\ECirc(-0.523727,-5.17909){0.542119}
\ECirc(29.9226,23.4405){0.706689}
\ECirc(-20.1843,60.841){0.400648}
\ECirc(2.62947,53.9421){0.685275}
\ECirc(-10.0203,-21.4844){0.647176}
\ECirc(-36.7819,-10.7662){0.600038}
\ECirc(-36.4626,-8.73091){2.10601}
\ECirc(30.3653,-25.2912){1.03241}
\ECirc(-1.24566,-3.59646){0.703128}
\ECirc(-9.90783,-8.32712){0.681608}
\ECirc(27.1758,5.33858){1.01049}
\ECirc(14.2366,-9.27061){0.761194}
\ECirc(6.39698,-0.497744){0.487311}
\ECirc(5.42717,2.7591){0.211982}
\ECirc(2.91016,2.58519){0.52981}
\ECirc(4.2632,-8.72988){0.838214}
\ECirc(24.9064,45.5064){0.512333}
\ECirc(41.6775,3.93545){1.08119}
\ECirc(27.6138,74.5208){1.30272}
\ECirc(5.10702,35.0652){0.692091}
\ECirc(9.6384,-3.68102){0.64568}
\ECirc(-27.4433,-3.83707){0.61559}
\ECirc(-29.3502,-3.13726){0.725784}
\ECirc(-26.3799,-3.09587){0.459014}
\ECirc(-30.5446,-5.1706){2.18432}
\ECirc(-6.12222,43.0524){0.716003}
\ECirc(-12.0524,41.5887){0.723929}
\ECirc(-13.6436,2.72484){0.691844}
\ECirc(12.8744,-51.3319){0.71508}
\ECirc(3.27875,-3.5693){0.394655}
\ECirc(4.64483,-2.8791){1.15894}
\ECirc(48.9494,27.9892){1.29084}
\ECirc(-26.8978,26.7142){0.952311}
\ECirc(11.3772,-48.9431){0.355879}
\ECirc(-37.0703,-40.158){1.06342}
\ECirc(18.0688,-6.91502){0.70329}
\ECirc(18.1953,27.1689){0.774623}
\ECirc(-12.833,-17.3661){0.704348}
\ECirc(-42.8978,-12.2025){0.682729}
\ECirc(24.5958,4.33884){0.753655}
\ECirc(37.9914,-1.77103){0.574104}
\ECirc(35.0797,-24.2798){0.463804}
\ECirc(49.1143,-0.635833){0.979429}
\ECirc(9.48033,56.3757){0.691354}
\ECirc(63.2465,17.3999){0.669167}
\ECirc(55.5185,-3.13136){0.966819}
\ECirc(55.6204,-2.90522){0.71115}
\ECirc(-26.1655,-16.2155){0.619369}
\ECirc(2.18654,-54.6451){0.67864}
\ECirc(-2.52337,-3.96904){0.575512}
\ECirc(-2.7207,-1.50994){0.746652}
\ECirc(-6.56223,34.1571){1.98842}
\ECirc(7.81052,-49.6388){0.676234}
\ECirc(64.4963,-18.0011){0.639323}
\ECirc(7.86455,29.584){0.773034}
\ECirc(52.1012,16.0242){1.28506}
\ECirc(56.3203,19.3464){1.58569}
\ECirc(51.8751,17.9852){0.705903}
\ECirc(26.7751,-11.1508){0.685469}
\ECirc(11.8191,39.8624){0.676154}
\ECirc(62.2514,-21.5548){1.05355}
\ECirc(-23.9528,-17.2333){0.534003}
\ECirc(42.2576,7.34202){0.822592}
\ECirc(-1.28418,51.9528){0.301653}
\ECirc(0.340675,-44.146){1.25302}
\ECirc(8.05512,3.07716){1.28569}
\ECirc(-12.7634,-7.555){0.681777}
\ECirc(-10.6481,-32.7847){0.278431}
\ECirc(-7.7075,-34.5333){0.340883}
\ECirc(-10.047,-34.5008){0.436406}
\ECirc(-9.72486,-27.6041){0.436088}
\ECirc(-10.9998,-40.1237){0.519318}
\ECirc(-36.0878,44.8753){0.625676}
\ECirc(23.088,0.697153){0.705273}
\ECirc(-32.7905,-0.567764){0.638812}
\ECirc(-42.4076,-2.06313){0.281831}
\ECirc(47.2153,30.1901){1.09776}
\ECirc(42.6963,29.7376){1.80547}
\ECirc(42.173,29.9069){3.7191}
\ECirc(20.9769,7.8884){1.63193}
\ECirc(-34.1384,14.7408){0.416747}
\ECirc(-36.1394,19.2053){1.04316}
\ECirc(-36.5582,17.9027){0.222893}
\ECirc(-37.0319,16.7509){0.197537}
\ECirc(-9.95327,-30.0007){0.396266}
\ECirc(51.3568,36.9907){0.370546}
\ECirc(50.8595,37.5387){0.473919}
\ECirc(-46.931,-9.26163){0.331374}
\ECirc(-46.0152,-7.46688){0.596573}
\ECirc(-25.9215,19.4554){1.51114}
\ECirc(-44.3296,-27.7563){0.603875}
\ECirc(-49.7391,-24.8459){1.7605}
\ECirc(44.414,-36.6209){0.553578}
\ECirc(-43.1143,33.9082){0.429664}
\ECirc(-23.844,-11.0661){0.861474}
\ECirc(-46.6116,-14.8366){0.925161}
\ECirc(15.8376,-55.912){0.268448}
\ECirc(15.6998,-54.6124){0.690488}
\ECirc(1.34053,15.6743){0.782467}
\ECirc(19.3489,-45.0746){0.510313}
\ECirc(18.5888,-44.5555){0.434049}
\ECirc(21.3793,58.6786){0.876627}
\ECirc(21.2882,60.1733){0.746243}
\ECirc(6.34324,5.40231){0.580606}
\ECirc(5.30319,10.4158){0.606378}
\ECirc(5.98915,-15.5762){0.705482}
\ECirc(-22.3203,16.7246){0.446035}
\ECirc(-2.85679,-15.2535){0.513424}
\ECirc(-0.948802,-17.4201){0.473273}
\ECirc(-4.38249,-12.1522){0.794682}
\ECirc(24.7495,-15.0572){0.582822}
\ECirc(3.28678,11.089){0.520277}
\ECirc(3.16965,-0.152246){1.23971}
\ECirc(-28.468,46.6683){0.508729}
\ECirc(-46.5676,-13.2341){0.684226}
\ECirc(-32.0914,-36.4858){0.319841}
\ECirc(3.86113,61.5214){0.669732}
\ECirc(10.8108,-47.1004){1.31252}
\ECirc(9.36419,-31.8338){0.571322}
\ECirc(7.94055,0.689409){0.707079}
\ECirc(62.6368,-18.8706){0.693507}
\ECirc(-31.5438,-45.7183){0.892532}
\ECirc(48.5613,30.5112){0.662285}
\ECirc(44.2186,32.5032){0.61961}
\ECirc(48.6303,-39.8721){0.797284}
\ECirc(49.7246,-36.8233){0.534956}
\ECirc(2.47099,12.7686){0.581382}
\ECirc(-47.6756,-11.8965){0.840299}
\ECirc(16.0423,-32.8015){0.698363}
\ECirc(18.9037,-33.011){0.722995}
\ECirc(19.9325,-31.3404){1.72389}
\ECirc(-12.1888,-21.5978){0.704573}
\ECirc(28.3258,32.0414){0.706855}
\ECirc(-13.97,1.31733){0.771529}
\ECirc(-42.5741,1.28354){0.613985}
\ECirc(58.4631,-3.22734){0.706283}
\ECirc(37.3917,-1.85603){0.954767}
\ECirc(37.7653,-2.68494){1.04302}
\ECirc(18.548,-12.5405){0.956018}
\ECirc(-36.0165,-5.89036){0.706728}
\ECirc(13.1499,-4.13296){0.697367}
\ECirc(-35.2874,17.7548){0.608507}
\ECirc(-34.0828,17.933){0.264585}
\ECirc(34.0727,-48.0544){0.657805}
\ECirc(-10.6392,8.59241){0.39298}
\ECirc(-11.8892,7.91145){0.370418}
\ECirc(-11.3513,7.18475){0.200646}
\ECirc(-17.0232,-18.8268){0.664521}
\ECirc(-35.8312,13.4043){0.513147}
\ECirc(-33.0003,11.2618){1.00817}
\ECirc(29.6452,27.3412){0.629886}
\ECirc(4.9364,1.84556){0.732784}
\ECirc(-18.274,-22.5672){1.23783}
\ECirc(9.43786,3.32262){0.695164}
\ECirc(25.0908,31.9916){0.822876}
\ECirc(2.85613,54.4667){0.720997}
\ECirc(-32.7286,4.84917){0.915825}
\ECirc(-32.4686,5.90888){0.715863}
\ECirc(0.786962,50.4284){0.529152}
\ECirc(-20.9757,-15.243){0.67422}
\ECirc(38.3847,-3.29873){0.533928}
\ECirc(38.5513,1.78108){0.285294}
\ECirc(-5.14294,46.3566){1.35966}
\ECirc(22.3623,23.6772){0.353134}
\ECirc(22.9432,20.1247){0.358617}
\ECirc(21.8914,23.8552){0.705713}
\ECirc(27.0997,24.0885){0.567638}
\ECirc(53.9553,38.3559){0.476951}
\ECirc(-16.9857,-18.712){0.436359}
\ECirc(-21.5532,-19.0658){0.399363}
\ECirc(-17.2393,2.80957){0.716546}
\ECirc(25.0931,-6.05938){0.68234}
\ECirc(22.2471,-21.8489){0.699189}
\ECirc(-50.5198,1.60571){0.735166}
\ECirc(-47.5992,2.2075){0.500441}
\ECirc(6.52304,-4.07326){0.399747}
\ECirc(12.4509,-1.00377){0.560718}
\ECirc(21.3306,-38.3353){0.706563}
\ECirc(7.88896,34.9058){0.430313}
\ECirc(6.12238,36.8095){0.42633}
\ECirc(-18.5804,13.5775){0.528151}
\ECirc(-27.6373,-22.1712){0.79248}
\ECirc(45.5286,-9.1551){0.476861}
\ECirc(45.5484,-9.84806){0.940059}
\ECirc(44.9126,-9.30517){0.560894}
\ECirc(46.013,-10.2725){0.679888}
\ECirc(-39.4895,-29.2448){0.674116}
\ECirc(-39.9166,-29.9972){0.572717}
\ECirc(-6.01351,-9.85954){0.435464}
\ECirc(21.0028,34.5478){1.71347}
\ECirc(20.3715,-38.5422){0.785081}
\ECirc(26.3273,-39.0115){0.675373}
\ECirc(28.0327,-35.6885){0.656368}
\ECirc(34.4709,29.7294){0.543106}
\ECirc(-7.87321,-0.0211631){0.693862}
\ECirc(13.7433,-19.0852){0.666955}
\ECirc(-27.741,47.3052){0.412795}
\ECirc(-27.7005,46.9779){0.552225}
\ECirc(-14.4125,-11.8668){0.738413}
\ECirc(7.19282,0.524387){0.68289}
\ECirc(26.8121,20.3818){1.25812}
\ECirc(-4.36601,-5.06176){0.487096}
\ECirc(49.4732,-13.7207){0.887626}
\ECirc(4.19426,-21.331){0.464708}
\ECirc(4.53167,-28.596){0.636602}
\ECirc(-10.1431,6.12134){0.760034}
\ECirc(14.3524,-49.6916){1.55346}
\ECirc(12.9046,-49.3765){0.547373}
\ECirc(12.4968,-50.5046){0.547654}
\ECirc(19.3199,-19.0271){0.647585}
\ECirc(22.0702,-24.3681){0.457048}
\ECirc(-44.3478,1.82781){0.706839}
\ECirc(9.26673,-24.9651){0.448724}
\ECirc(3.64485,-28.0952){0.702463}
\ECirc(4.72386,-26.6316){0.47757}
\ECirc(11.0926,-30.2879){1.24426}
\ECirc(12.3404,-2.40311){0.705191}
\ECirc(33.7279,-46.635){0.937909}
\ECirc(30.0874,-42.2795){1.11434}
\ECirc(-7.90976,-37.5692){0.705765}
\ECirc(3.68099,17.5306){0.504754}
\ECirc(12.3072,-27.396){0.707077}
\ECirc(11.2381,-24.2263){0.602031}
\ECirc(17.6431,-25.3788){0.884541}
\ECirc(15.1856,-21.8336){0.3946}
\ECirc(-5.8717,-58.1041){0.706956}
\ECirc(41.2159,3.1588){0.702244}
\ECirc(40.8802,3.62974){0.51635}
\ECirc(42.8465,4.03227){0.35864}
\ECirc(-33.8681,-26.8572){0.804933}
\ECirc(4.50985,-13.6622){1.47033}
\ECirc(15.8723,-55.1076){0.847751}
\ECirc(-1.70153,25.9581){0.640041}
\ECirc(-35.3535,-0.473066){0.575669}
\ECirc(16.9255,-8.6913){0.496155}
\ECirc(15.9055,-8.37924){4.73904}
\ECirc(19.8565,-12.7737){0.598764}
\ECirc(33.0505,29.9555){0.701634}
\ECirc(33.2925,30.2137){0.810945}
\ECirc(46.8068,-10.8631){1.28808}
\ECirc(-11.6681,45.3773){0.700096}
\ECirc(-12.2201,-31.1466){1.19624}
\ECirc(0.194087,-4.16299){0.687899}
\ECirc(3.69746,-3.94792){0.775237}
\ECirc(58.231,-9.28674){0.750616}
\ECirc(-14.2926,-56.1601){1.73409}
\ECirc(-43.7414,39.3749){2.05255}
\ECirc(-47.683,37.3604){1.25752}
\ECirc(-47.5813,38.1253){1.38907}
\ECirc(-47.8101,33.3443){0.689066}
\ECirc(-7.18306,-5.70459){0.757857}
\ECirc(28.0847,29.044){0.686024}
\ECirc(35.0047,-41.2661){0.957139}
\ECirc(41.8999,-43.2496){1.31797}
\ECirc(42.6143,-43.1525){0.62259}
\ECirc(1.42208,25.8404){0.701245}
\ECirc(-6.91665,-36.3198){0.706576}
\ECirc(15.5119,-3.34251){1.397}
\ECirc(-15.0337,-35.7123){0.705071}
\ECirc(29.0629,20.3985){0.706601}
\ECirc(56.3195,-0.303516){0.56927}
\ECirc(58.4585,0.816125){0.677894}
\ECirc(59.1296,1.65096){0.654427}
\ECirc(7.16624,8.52645){0.787538}
\ECirc(-20.3487,-18.6463){1.09214}
\ECirc(-2.91522,7.54364){0.690183}
\ECirc(-1.63435,0.121613){0.70647}
\ECirc(58.2704,-11.831){0.645729}
\ECirc(-23.5742,5.47797){0.191184}
\ECirc(-22.7759,5.54998){0.313871}
\ECirc(-38.3876,-30.9697){0.700482}
\ECirc(-29.5698,-5.2492){3.5867}
\ECirc(18.3476,-3.84904){0.541066}
\ECirc(54.8144,43.5651){0.70245}
\ECirc(52.6601,44.6757){0.610027}
\ECirc(6.98146,-15.3582){1.00406}
\ECirc(-48.0845,11.4724){1.05985}
\ECirc(-38.569,38.3665){0.526416}
\ECirc(-40.8345,0.869018){0.68984}
\ECirc(-42.4866,0.0694257){1.41251}
\ECirc(50.2292,43.6459){0.703225}
\ECirc(-31.1439,29.3123){0.407044}
\ECirc(3.80984,-2.29457){1.1534}
\ECirc(12.2851,2.54923){1.06587}
\ECirc(13.433,5.14686){0.850011}
\ECirc(21.9477,14.0459){0.326768}
\ECirc(-6.43382,-37.9261){0.69573}
\ECirc(-10.5335,-13.1994){0.401237}
\ECirc(-6.30431,-16.7079){0.878622}
\ECirc(-42.9286,-16.0462){0.832786}
\ECirc(-28.7612,-29.7874){0.563262}
\ECirc(-2.20668,-18.883){0.695912}
\ECirc(-30.9271,-19.5138){0.72362}
\ECirc(53.9703,14.1256){0.829207}
\ECirc(-13.5901,-55.9201){0.749948}
\ECirc(-19.4372,57.824){0.476014}
\ECirc(-1.33702,-18.4952){0.299162}
\ECirc(-3.94156,-5.77528){1.31989}
\ECirc(-14.4129,-3.6861){0.681411}
\ECirc(-8.40355,-5.44429){0.67355}
\ECirc(45.2431,29.4313){0.691957}
\ECirc(-14.6063,-54.0365){0.956818}
\ECirc(25.0533,35.3582){0.706914}
\ECirc(44.4912,-14.7444){0.534868}
\ECirc(44.8588,-9.66715){0.577713}
\ECirc(50.6776,-12.6041){0.381686}
\ECirc(46.7505,-17.3382){0.43248}
\ECirc(47.0478,-9.68733){0.650384}
\ECirc(51.7165,-11.1938){1.00115}
\ECirc(51.9664,-14.1594){0.649207}
\ECirc(49.7128,-14.2901){0.713578}
\ECirc(10.9974,-2.75919){0.703582}
\ECirc(8.63906,6.83557){0.310045}
\ECirc(-53.4422,33.3799){0.812888}
\ECirc(-12.0538,4.08195){0.913405}
\ECirc(-43.2939,7.12338){0.824056}
\ECirc(21.4239,29.3656){0.533764}
\ECirc(23.3855,35.5877){0.868873}
\ECirc(18.6709,35.4369){0.539275}
\ECirc(22.7497,36.6601){0.511673}
\ECirc(-53.0874,-18.2237){0.441784}
\ECirc(-54.2809,-20.8473){0.413822}
\ECirc(-48.0822,-17.2684){0.520922}
\ECirc(-12.0797,-20.4744){0.898524}
\ECirc(20.8146,-38.4196){0.667379}
\ECirc(43.1723,-3.28427){0.681372}
\ECirc(6.28558,-47.1302){0.707067}
\ECirc(8.42005,-56.2719){0.606677}
\ECirc(-58.0743,20.5271){0.809038}
\ECirc(-59.9024,18.9475){0.491644}
\ECirc(-11.3121,7.06227){0.703618}
\ECirc(-0.762067,16.2777){0.611546}
\ECirc(1.59621,14.9267){0.696613}
\ECirc(-9.00393,47.9353){0.622838}
\ECirc(-10.7085,45.8698){0.307463}
\ECirc(-25.6644,35.1042){0.688581}
\ECirc(-26.5897,36.0662){0.518873}
\ECirc(22.3079,-39.1981){0.548967}
\ECirc(-15.5263,-44.0386){0.538579}
\ECirc(-7.34779,-43.7103){0.637111}
\ECirc(36.3374,39.8131){0.779126}
\ECirc(12.6178,-43.5759){0.702668}
\ECirc(4.24271,-17.6099){0.832338}
\ECirc(41.0601,24.1627){0.523828}
\ECirc(-11.9676,-21.6027){0.706955}
\ECirc(-28.73,32.0003){1.22855}
\ECirc(-46.3695,-8.23009){0.712634}
\ECirc(-22.6229,17.6611){0.461487}
\ECirc(-22.3989,22.5144){0.363201}
\ECirc(37.348,-2.35618){1.00351}
\ECirc(38.1928,-4.28729){0.678249}
\ECirc(-45.5217,-27.2825){1.2905}
\ECirc(-35.3557,43.9624){0.700656}
\ECirc(53.718,35.2007){0.70317}
\ECirc(-56.9254,36.367){1.00717}
\ECirc(61.7263,18.418){0.714139}
\ECirc(51.5511,40.7458){0.70663}
\ECirc(17.5808,23.197){1.03398}
\ECirc(14.5733,-57.1304){0.707068}
\ECirc(-53.6358,4.26077){0.812914}
\ECirc(-2.58021,0.290945){2.15623}
\ECirc(0.323119,0.0218387){1.02375}
\ECirc(2.12994,1.41152){0.618715}
\ECirc(-6.0925,24.8679){0.661969}
\ECirc(-6.08968,29.8759){0.945578}
\ECirc(21.9743,-12.0427){0.706393}
\ECirc(-22.2455,18.9933){1.30926}
\ECirc(-22.3174,5.14938){0.650727}
\ECirc(17.9947,30.1615){0.47207}
\ECirc(15.4004,26.2929){0.698384}
\ECirc(-18.3324,-16.1394){0.707042}
\ECirc(-25.8896,4.67786){0.67978}
\ECirc(-19.4817,18.8221){0.755431}
\ECirc(49.4778,-17.8988){0.688614}
\ECirc(31.4592,-28.5857){0.545737}
\ECirc(-12.1853,-39.9132){0.707007}
\ECirc(-38.8959,17.3898){0.658949}
\ECirc(31.5176,9.78904){0.69447}
\ECirc(-18.0535,-50.3555){0.677275}
\ECirc(-19.8091,10.5235){0.69601}
\ECirc(-26.8419,3.72017){0.787833}
\ECirc(-23.4676,5.83846){0.705683}
\ECirc(-27.3192,4.66057){0.447922}
\ECirc(6.07636,-23.4858){1.44345}
\ECirc(-26.8893,-8.27682){0.319473}
\ECirc(54.0604,-9.94321){0.704708}
\ECirc(-11.0293,-5.17406){0.697343}
\ECirc(-48.1087,6.55846){5}
\ECirc(-3.32295,44.4924){0.705979}
\ECirc(-23.3938,18.0173){0.50078}
\ECirc(-21.3566,21.9258){1.3753}
\ECirc(-10.5611,-38.5985){1.47889}
\ECirc(1.66674,-2.27521){1.01453}
\ECirc(13.1285,5.69444){0.627887}
\ECirc(15.9338,6.18663){0.320316}
\ECirc(16.1433,6.44993){0.313815}
\ECirc(13.6635,3.73076){1.23903}
\ECirc(-21.5304,-6.0776){2.28018}
\ECirc(-37.1673,42.335){1.01334}
\ECirc(-39.1183,44.3799){0.503452}
\ECirc(-34.3946,42.2523){1.09971}
\ECirc(22.5997,14.0544){0.702112}
\ECirc(26.4259,13.7745){1.35954}
\ECirc(36.6382,-38.279){2.25133}
\ECirc(-48.1924,39.4177){0.420848}
\ECirc(18.5286,-35.1761){0.7054}
\ECirc(42.4993,8.79784){0.526491}
\ECirc(43.1037,9.05732){0.589324}
\ECirc(43.596,8.11254){0.689954}
\ECirc(45.8831,0.330919){0.666515}
\ECirc(-8.82239,-5.50701){0.737849}
\ECirc(-35.301,-14.5277){1.2105}
\ECirc(36.3281,-29.9999){0.707075}
\ECirc(-65.9168,5.59617){1.13235}
\ECirc(-51.3232,30.4434){1.71565}
\ECirc(-48.9988,32.8408){0.898927}
\ECirc(-48.5247,35.1102){1.14909}
\ECirc(-52.7579,23.7714){0.771405}
\ECirc(-55.4541,20.1056){0.647655}
\ECirc(18.029,-39.1688){0.706896}
\ECirc(-23.7875,47.2701){0.622058}
\ECirc(-30.2922,45.6191){0.892557}
\ECirc(-31.2989,47.3228){0.848534}
\ECirc(44.6131,-35.4944){0.387606}
\ECirc(48.3162,-35.9109){0.497137}
\ECirc(48.2735,-34.2484){0.264488}
\ECirc(49.5105,-38.8393){0.584624}
\ECirc(4.99809,-10.9476){0.52071}
\ECirc(4.51961,-10.195){1.76135}
\ECirc(5.46268,-9.5521){1.82517}
\ECirc(7.23016,-10.718){0.555856}
\ECirc(7.15684,-11.4675){0.625225}
\ECirc(9.65094,-5.34702){0.953548}
\ECirc(18.2934,-13.2646){0.352752}
\ECirc(21.4771,-12.5815){0.394241}
\ECirc(51.7228,-28.9311){0.703708}
\ECirc(49.1664,-33.4767){0.430535}
\ECirc(49.4232,-33.3653){0.439234}
\ECirc(48.3395,-31.296){0.342722}
\ECirc(6.56234,6.69184){0.683657}
\ECirc(8.98704,-0.0863279){0.716252}
\ECirc(-31.076,-17.9063){0.73468}
\ECirc(-16.7897,-45.3324){0.352466}
\ECirc(-15.6219,-44.1377){1.02034}
\ECirc(-13.0926,-46.8719){0.405035}
\ECirc(-14.3795,-45.2034){0.555228}
\ECirc(24.1675,-23.6822){0.675589}
\ECirc(-28.7665,20.9007){0.742272}
\ECirc(-9.52674,-23.1313){0.611323}
\ECirc(-28.0168,30.4749){0.701953}
\ECirc(16.8584,-32.9704){0.704268}
\ECirc(7.72051,-31.8977){0.709591}
\ECirc(7.11091,-29.9394){0.703409}
\ECirc(-20.2437,12.8491){0.703545}
\ECirc(-20.7039,13.1011){0.72234}
\ECirc(-56.7912,-28.5749){0.699959}
\ECirc(12.0261,-35.8184){0.706847}
\ECirc(31.6459,35.909){0.680523}
\ECirc(10.4055,-49.2144){0.705705}
\ECirc(15.2091,-49.7779){0.706754}
\ECirc(-24.2104,30.8056){0.674187}
\ECirc(-30.4878,35.6348){0.702542}
\ECirc(-30.6155,35.8639){0.491576}
\ECirc(-32.5893,33.8669){0.348759}
\ECirc(22.6083,66.2237){0.569006}
\ECirc(21.5715,66.7717){0.739933}
\ECirc(21.021,67.2628){0.467001}
\ECirc(20.9741,-42.0927){0.70708}
\ECirc(-16.7811,-11.6162){0.706843}
\ECirc(27.14,31.0411){1.65788}
\ECirc(55.1971,41.3248){0.364532}
\ECirc(38.3127,28.0348){0.705736}
\ECirc(44.5188,30.6892){0.621894}
\ECirc(47.4013,-25.2048){0.683934}
\ECirc(20.1332,30.6197){0.706955}
\ECirc(23.1531,28.8978){0.883017}
\ECirc(-9.3357,9.70641){0.494739}
\ECirc(-9.4929,9.39698){0.208694}
\ECirc(-9.93413,11.3197){0.312366}
\ECirc(11.4899,-26.8509){0.768672}
\ECirc(11.2784,-23.9143){0.555069}
\ECirc(10.693,-24.9046){0.67942}
\ECirc(10.6567,-25.1529){0.723499}
\ECirc(-25.8249,-21.8511){0.70708}
\ECirc(8.83671,-62.1539){0.706844}
\ECirc(12.8452,-1.21826){0.56311}
\ECirc(20.4073,-26.2448){0.529684}
\ECirc(20.3741,-27.1052){0.944809}
\ECirc(53.3811,37.3479){0.313012}
\ECirc(52.9709,35.0768){0.815133}
\ECirc(31.9173,10.6246){0.645779}
\ECirc(-36.4426,16.6526){0.982527}
\ECirc(42.1755,9.76283){0.656342}
\ECirc(36.0476,12.1336){0.728743}
\ECirc(37.3937,12.7792){0.898366}
\ECirc(-15.7733,-29.2977){1.17844}
\ECirc(-15.7486,-29.3033){0.700411}
\ECirc(-44.8552,-10.4915){0.706542}
\ECirc(7.58589,-33.5901){1.13246}
\ECirc(-6.24796,-12.6345){0.706642}
\ECirc(-13.0505,-6.92551){0.408069}
\ECirc(-9.45335,-0.961071){0.550725}
\ECirc(-7.09064,-4.36859){0.678698}
\ECirc(-12.5552,-0.533119){0.873294}
\ECirc(-9.47209,-37.866){1.39453}
\ECirc(-11.7656,-38.5563){0.664067}
\ECirc(43.4694,-10.14){0.706801}
\ECirc(44.6945,-10.8051){0.622672}
\ECirc(-10.3583,-0.812273){0.408934}
\ECirc(-36.1262,4.20031){0.724537}
\ECirc(-38.9907,2.90331){0.942816}
\ECirc(-41.0936,-3.23092){0.59733}
\ECirc(-16.9553,23.1935){0.855263}
\ECirc(-14.0193,24.2032){0.465911}
\ECirc(-53.02,28.817){0.798939}
\ECirc(-54.3274,31.6093){0.703792}
\ECirc(63.9307,-21.1889){0.457114}
\ECirc(-24.7945,-4.06734){0.692623}
\ECirc(-16.7367,-8.37561){0.731837}
\ECirc(-21.5477,-5.13584){1.2562}
\ECirc(-21.6078,-3.83687){0.214002}
\ECirc(24.1893,-38.7441){1.26223}
\ECirc(23.1335,-40.5137){0.260687}
\ECirc(21.7439,-40.8665){0.271525}
\ECirc(-47.7479,38.1591){0.706764}
\ECirc(-10.4623,10.7515){0.349409}
\ECirc(-33.8598,12.4467){1.20163}
\ECirc(41.9726,-34.5658){0.70453}
\ECirc(52.4786,-31.9344){0.499349}
\ECirc(8.22753,-45.7709){1.00016}
\ECirc(-19.4255,-6.76128){0.637989}
\ECirc(-18.9067,-7.23339){0.618893}
\ECirc(-20.5622,-13.2468){0.448781}
\ECirc(-20.8826,-11.645){0.424452}
\ECirc(-14.5421,-15.9699){0.706736}
\ECirc(61.7071,-10.3807){0.706613}
\ECirc(-38.7094,-1.89248){0.303473}
\ECirc(6.80902,-0.530207){0.826222}
\ECirc(-16.4602,-33.1686){0.707089}
\ECirc(6.57864,36.242){0.707037}
\ECirc(5.79218,38.0043){0.465864}
\ECirc(67.9484,-20.1606){0.706674}
\ECirc(-53.1307,8.37686){0.701229}
\ECirc(-19.4063,-19.1297){0.720548}
\ECirc(11.765,-51.0243){0.698974}
\ECirc(9.70977,-50.9283){0.527314}
\ECirc(19.3371,-55.8072){0.707074}
\ECirc(-40.7697,43.4459){0.594176}
\ECirc(-37.5206,41.6929){0.580673}
\ECirc(42.5704,38.1711){0.668968}
\ECirc(-33.763,14.5632){1.42428}
\ECirc(-50.5175,33.3749){0.696045}
\ECirc(-6.12421,-38.3864){0.919372}
\ECirc(-4.50638,-35.2322){0.786761}
\ECirc(-4.99097,-40.1522){0.77968}
\ECirc(-1.09671,-1.07209){0.697018}
\ECirc(-59.9743,14.3033){0.710411}
\ECirc(48.8292,-32.5157){0.818335}
\ECirc(46.4555,-36.3274){0.477902}
\ECirc(46.4037,-35.2037){0.936505}
\ECirc(-15.194,1.70348){0.704224}
\ECirc(30.8601,-40.4829){0.706395}
\ECirc(29.4588,-41.1735){0.475937}
\ECirc(29.1367,-40.5518){0.527432}
\ECirc(-30.1606,11.2758){0.529561}
\ECirc(-56.9835,18.755){0.706918}
\ECirc(46.6224,36.4079){0.70692}
\ECirc(42.4318,30.7505){0.661122}
\ECirc(18.0164,42.9843){1.11731}
\ECirc(9.36505,-47.9836){0.810795}
\ECirc(-50.1005,9.39828){0.539527}
\ECirc(-51.2023,24.9143){0.721892}
\ECirc(-55.5777,22.343){0.333306}
\ECirc(-51.7626,21.6963){0.90026}
\ECirc(-50.314,21.8611){1.50758}
\ECirc(-8.78797,-23.4551){0.72542}
\ECirc(8.42581,-52.268){0.576005}
\ECirc(-39.2223,-12.644){0.766193}
\ECirc(-39.0281,-8.25906){0.706911}
\ECirc(-54.1835,25.7722){1.03798}
\ECirc(-14.0477,-51.5893){0.873588}
\ECirc(6.37708,-38.4129){0.707211}
\ECirc(-22.7706,18.6212){0.706992}
\ECirc(-32.975,-28.8629){0.368389}
\ECirc(-26.476,-31.9774){0.570984}
\ECirc(-31.7503,-21.2473){0.42456}
\ECirc(5.91371,-12.2929){0.549477}
\ECirc(1.73535,-30.4536){0.895515}
\ECirc(-12.196,27.7826){0.69199}
\ECirc(-13.3586,29.8406){0.866145}
\ECirc(-47.8258,26.7832){1.58361}
\ECirc(6.34223,8.6384){0.776197}
\ECirc(7.7827,-49.1886){0.675744}
\ECirc(-31.3954,4.27834){1.88659}
\ECirc(21.2108,-17.3334){0.442181}
\ECirc(22.8019,-9.14492){0.381918}
\ECirc(24.7172,-11.7327){0.428336}
\ECirc(-6.58933,-17.1394){0.892275}
\ECirc(0.82371,3.5128){0.732365}
\ECirc(9.55604,3.1585){0.796621}
\ECirc(15.6789,28.6409){0.754735}
\ECirc(2.05673,29.632){1.68446}
\ECirc(-12.7667,39.3157){0.708831}
\ECirc(-20.407,43.499){0.965985}
\ECirc(-6.74093,39.0232){1.45794}
\ECirc(44.2286,-36.78){0.258785}
\ECirc(-10.7985,-7.11891){0.707097}
\ECirc(-55.9206,16.5822){1.32884}
\ECirc(-33.9421,-6.60541){0.706065}
\ECirc(5.15533,25.9537){0.707065}
\ECirc(46.8046,-50.4464){1.61405}
\ECirc(-7.75622,24.9){0.706822}
\ECirc(47.613,13.4714){0.949166}
\ECirc(10.1251,-35.5815){0.587591}
\ECirc(5.61741,-35.1536){0.552972}
\ECirc(-7.36238,-52.179){0.448613}
\ECirc(-6.48752,-50.7141){0.621196}
\ECirc(-6.44657,-50.5101){0.670993}
\ECirc(-7.16226,-51.138){0.707837}
\ECirc(-4.10298,-50.7522){0.607784}
\ECirc(-3.42795,-53.3628){0.707075}
\ECirc(10.2474,-47.9867){1.01571}
\ECirc(10.7542,-49.3577){0.516322}
\ECirc(13.6005,-51.4557){0.65881}
\ECirc(15.3582,-49.1239){0.340276}
\ECirc(13.5077,-19.2317){0.707085}
\ECirc(-22.1868,-24.8067){0.707061}
\ECirc(-4.86422,1.70282){0.9281}
\ECirc(46.2676,30.4724){0.939029}
\ECirc(1.96904,52.9075){0.706884}
\ECirc(46.956,-10.133){0.706894}
\ECirc(21.2538,-0.367073){0.792638}
\ECirc(-46.4668,-7.98919){0.407542}
\ECirc(-46.7604,-9.96608){0.247255}
\ECirc(-47.2667,-11.3188){0.574476}
\ECirc(-23.5171,31.665){0.503024}
\ECirc(-25.4048,32.9978){0.499356}
\ECirc(-21.3261,42.1343){0.650629}
\ECirc(61.5509,-17.5449){1.4991}
\ECirc(3.48239,-3.65504){0.69549}
\ECirc(0.81968,17.3792){0.664384}
\ECirc(1.97315,17.8008){0.70541}
\ECirc(-39.7136,-6.82051){0.706362}
\ECirc(41.489,2.8436){0.706612}
\ECirc(25.6114,27.5391){0.608151}
\ECirc(-2.20341,-25.6099){1.39734}
\ECirc(21.1694,-10.8872){0.706998}
\ECirc(-3.12935,20.565){0.694848}
\ECirc(-38.6923,2.54455){0.90966}
\ECirc(-40.1499,8.55276){0.739217}
\ECirc(9.77885,-6.08958){0.707092}
\ECirc(-6.23655,-9.65166){0.707077}
\ECirc(-17.0321,7.79689){0.485475}
\ECirc(-15.4337,-11.8256){1.05411}
\ECirc(26.6515,-12.686){0.781819}
\ECirc(-22.9141,-22.1819){1.78165}
\ECirc(-35.3132,-35.3353){0.706774}
\ECirc(-30.1462,36.305){0.795962}
\ECirc(19.4678,-7.67729){0.257352}
\ECirc(16.0829,-7.76364){1.03671}
\ECirc(26.3955,-10.855){0.373883}
\ECirc(27.9301,-12.0493){0.49458}
\ECirc(28.9484,-9.76128){0.857285}
\ECirc(8.36204,-23.3717){1.30273}
\ECirc(8.64051,-27.5635){1.37977}
\ECirc(13.4018,-23.8329){0.638261}
\ECirc(9.05317,-26.0963){0.706734}
\ECirc(6.88516,35.8505){0.974316}
\ECirc(3.59875,31.6629){0.974316}
\ECirc(2.73744,33.5347){0.435086}
\ECirc(2.59289,33.8902){0.691208}
\ECirc(9.79409,-53.5422){1.19166}
\ECirc(10.7825,-21.2729){0.707101}
\ECirc(-27.8119,-11.8123){0.707035}
\ECirc(-0.478503,53.9002){1.33932}
\ECirc(-3.10385,15.3293){0.794077}
\ECirc(-0.713584,18.0269){2.38016}
\ECirc(-45.7683,25.1649){2.68533}
\ECirc(-46.5161,24.3113){0.773994}
\ECirc(-46.5276,25.5962){2.14128}
\ECirc(-46.3569,26.4256){0.26706}
\ECirc(-47.0366,26.2522){0.246255}
\ECirc(-16.633,-9.88058){0.707082}
\ECirc(-22.8317,19.373){1.2296}
\ECirc(-28.8809,15.5141){0.315613}
\ECirc(-25.6285,17.2426){0.429916}
\ECirc(22.3827,-38.2294){0.556198}
\ECirc(5.17427,31.888){0.703755}
\ECirc(2.80732,32.0736){0.445814}
\ECirc(2.55764,31.6256){0.328953}
\ECirc(2.73658,31.2043){0.328953}
\ECirc(22.0484,24.6189){0.940238}
\ECirc(19.725,24.1066){0.706654}
\ECirc(22.3551,31.2095){0.450283}
\ECirc(-40.4947,-30.7228){0.725653}
\ECirc(-39.3634,-0.279774){0.663808}
\ECirc(-0.807243,2.23688){0.701869}
\ECirc(24.9632,34.3835){0.990424}
\ECirc(22.9865,31.2301){0.517242}
\ECirc(-32.891,-15.0286){3.05063}
\ECirc(-5.13846,-15.7102){0.74709}
\ECirc(34.8564,-27.6523){0.666362}
\ECirc(-42.2247,-28.1339){1.26487}
\ECirc(-46.0572,-21.1108){0.864772}
\ECirc(-1.32327,-14.6851){0.61392}
\ECirc(22.8043,44.2809){0.706651}
\ECirc(-33.8666,37.8798){0.705925}
\ECirc(15.4267,6.38215){2.2962}
\ECirc(54.1707,10.606){0.551978}
\ECirc(57.0873,11.2169){0.555331}
\ECirc(52.2216,11.8725){0.994799}
\ECirc(-37.3816,31.0439){1.19765}
\ECirc(-27.8709,29.986){0.819923}
\ECirc(0.12259,52.9438){0.488481}
\ECirc(1.46708,53.6563){0.592882}
\ECirc(1.81946,53.7384){0.85918}
\ECirc(-3.40191,53.2449){0.332116}
\ECirc(-1.21667,54.9906){0.647243}
\ECirc(10.9545,-25.6092){0.707104}
\ECirc(41.9468,-13.5289){0.803051}
\ECirc(14.4083,7.37747){0.715182}
\ECirc(-17.1478,6.75666){0.70708}
\ECirc(-9.44681,-3.22737){0.352993}
\ECirc(5.34211,33.9177){0.702845}
\ECirc(31.3249,-24.9721){0.795462}
\ECirc(15.9854,-35.9308){0.713168}
\ECirc(13.7997,-49.2235){1.01077}
\ECirc(44.1714,4.92652){0.796176}
\ECirc(42.4742,7.19814){0.633027}
\ECirc(-26.3855,51.2063){0.295178}
\ECirc(-25.8446,50.5946){1.11402}
\ECirc(4.74573,-0.979274){0.736915}
\ECirc(-12.2526,26.4374){0.580396}
\ECirc(-15.1895,25.6068){0.434294}
\ECirc(-17.9674,28.5557){0.887346}
\ECirc(-18.6107,23.9972){0.887105}
\ECirc(-9.00232,68.2007){0.634259}
\ECirc(7.16484,-58.9498){0.707067}
\ECirc(-11.9267,5.25015){0.399713}
\ECirc(1.89755,5.0979){1.52577}
\ECirc(-38.2722,-8.24533){0.64659}
\ECirc(-43.445,-9.78882){0.375526}
\ECirc(-32.4571,-8.33605){0.949105}
\ECirc(28.2428,11.8467){1.28486}
\ECirc(55.2749,41.7458){1.64022}
\ECirc(60.2379,27.2024){0.678956}
\ECirc(53.8788,17.7126){0.685739}
\ECirc(-8.97429,46.7205){1.12867}
\ECirc(-10.5069,46.9462){0.840318}
\ECirc(-10.4833,47.3823){0.480872}
\ECirc(23.6501,-11.0798){0.706969}
\ECirc(-37.339,-1.87077){0.462621}
\ECirc(1.80659,22.3473){1.10656}
\ECirc(2.33172,-15.1676){1.54681}
\ECirc(8.98813,-16.8446){0.498313}
\ECirc(8.0998,-9.79921){1.12071}
\ECirc(43.0213,-23.0705){2.04249}
\ECirc(58.1253,-8.73648){0.457842}
\ECirc(60.3208,-9.57918){0.467397}
\ECirc(58.8766,-11.2354){0.395834}
\ECirc(-15.1758,-13.8161){0.706818}
\ECirc(-22.7692,50.4094){1.20401}
\ECirc(-22.1888,49.7057){0.632803}
\ECirc(-22.0852,53.4653){0.705913}
\ECirc(-3.95536,-60.3455){0.887663}
\ECirc(-1.58746,-61.6582){0.748063}
\ECirc(0.436244,-58.3847){0.472073}
\ECirc(3.65273,-60.0139){0.350735}
\ECirc(-46.2859,-15.8743){1.23273}
\ECirc(-25.5665,33.831){0.486519}
\ECirc(24.866,45.4188){1.10233}
\ECirc(-10.4523,-24.4489){0.494413}
\ECirc(-44.0554,-13.9947){0.703454}
\ECirc(-39.3298,-15.7705){1.17621}
\ECirc(10.9527,-25.1114){0.881413}
\ECirc(-39.5473,21.2653){0.705706}
\ECirc(-29.931,31.8362){0.525704}
\ECirc(-37.6788,27.0216){0.389806}
\ECirc(13.7277,23.4378){0.78554}
\ECirc(15.0809,22.4146){0.518626}
\ECirc(14.6786,22.9398){0.465825}
\ECirc(-1.39917,-18.371){0.707017}
\ECirc(-3.7366,23.2343){0.490268}
\ECirc(-5.59729,27.6556){0.551191}
\ECirc(-7.83313,27.509){0.344259}
\ECirc(-40.9711,-15.296){0.522311}
\ECirc(-41.0652,-7.58614){0.707091}
\ECirc(-41.6035,-9.00237){0.629332}
\ECirc(-41.3299,-8.20034){0.438978}
\ECirc(-37.9189,-8.79395){0.304419}
\ECirc(-41.9274,-7.38689){0.304419}
\ECirc(3.09736,-1.63842){0.433502}
\ECirc(-3.31781,12.6737){1.43577}
\ECirc(-3.70042,12.1272){0.575098}
\ECirc(-3.6712,15.4261){0.542861}
\ECirc(-2.61402,14.8436){0.465905}
\ECirc(68.0163,-15.9612){0.691083}
\ECirc(2.68575,28.4628){0.585496}
\ECirc(-12.6561,0.288299){0.707566}
\ECirc(-5.02405,-3.83903){1.00217}
\ECirc(-28.194,45.7549){0.606683}
\ECirc(-27.3327,38.8595){0.706534}
\ECirc(-1.83735,-57.4507){0.707077}
\ECirc(7.4843,-4.25715){0.707034}
\ECirc(-26.8971,46.7132){0.707049}
\ECirc(-23.0622,49.3183){0.517517}
\ECirc(-23.8486,47.7532){1.16928}
\ECirc(-29.4994,45.5309){0.557859}
\ECirc(13.6984,-4.91932){0.83304}
\ECirc(6.52897,-2.08777){0.690309}
\ECirc(8.11544,1.66339){0.982365}
\ECirc(-6.80066,30.3435){0.701434}
\ECirc(-7.15511,30.3017){0.529079}
\ECirc(-6.1951,34.4724){0.575814}
\ECirc(-13.9599,29.3179){0.95526}
\ECirc(-4.51905,32.5602){0.384721}
\ECirc(-6.89498,19.9083){0.706254}
\ECirc(-7.40999,19.3017){0.422204}
\ECirc(-39.2836,15.7593){0.701786}
\ECirc(-1.0573,16.6921){0.717294}
\ECirc(29.569,45.2518){0.479568}
\ECirc(22.6073,43.0998){0.815853}
\ECirc(22.9256,43.4057){1.37408}
\ECirc(22.891,47.7853){0.841481}
\ECirc(21.0161,-33.0279){0.506151}
\ECirc(-15.5958,-24.6465){0.517704}
\ECirc(-27.4773,-11.032){0.488447}
\ECirc(-18.1081,-18.6869){0.575244}
\ECirc(-23.3872,58.1643){0.707096}
\ECirc(-17.4526,-25.4118){0.707068}
\ECirc(37.0969,31.538){0.405381}
\ECirc(38.3784,33.3502){0.689449}
\ECirc(6.32437,-29.6391){0.440235}
\ECirc(7.09205,-18.9904){0.465873}
\ECirc(7.8655,-16.0185){1.01794}
\ECirc(9.95823,-17.8202){0.557645}
\ECirc(7.56877,-13.8122){0.707069}
\ECirc(59.776,-2.83104){0.338067}
\ECirc(56.0105,-0.517929){0.707017}
\ECirc(18.9824,-20.1254){0.427339}
\ECirc(-30.3345,-8.73671){1.22159}
\ECirc(-24.3569,-21.243){0.645619}
\ECirc(-10.3016,25.6174){0.983601}
\ECirc(-12.265,23.5416){0.684047}
\ECirc(-47.2304,46.4392){0.434111}
\ECirc(-49.3661,44.2031){0.521026}
\ECirc(-34.5387,30.4143){0.707087}
\ECirc(-2.81219,-2.67767){1.46141}
\ECirc(0.602241,-1.51056){0.979808}
\ECirc(5.75516,-0.731569){0.979455}
\ECirc(48.1175,16.8068){0.706924}
\ECirc(-52.9471,-19.4049){1.10912}
\ECirc(-29.7882,6.83997){0.990395}
\ECirc(-35.9626,3.70669){0.962336}
\ECirc(-38.2556,3.94105){0.788695}
\ECirc(-37.6481,2.23856){0.527762}
\ECirc(-11.0811,6.06572){0.690704}
\ECirc(-11.8831,3.59039){0.690704}
\ECirc(-12.1938,4.78584){1.11941}
\ECirc(8.65637,8.03859){0.663288}
\ECirc(5.58298,38.547){0.707081}
\ECirc(3.84159,34.8519){0.404715}
\ECirc(2.39003,35.3406){0.221593}
\ECirc(2.39908,36.7458){0.271825}
\ECirc(-20.0866,-36.7916){0.402066}
\ECirc(-20.6058,-38.4974){0.419959}
\ECirc(-21.7965,-36.6503){0.477469}
\ECirc(21.4394,24.7456){0.430287}
\ECirc(-4.59237,-42.9336){0.696563}
\ECirc(-9.14038,-43.2003){0.476201}
\ECirc(-52.728,23.1849){0.706991}
\ECirc(-23.5027,-23.5422){0.333731}
\ECirc(-26.8043,-26.4817){0.503118}
\ECirc(-34.1504,-13.1027){0.646466}
\ECirc(42.2669,29.2744){0.456196}
\ECirc(20.3662,4.17387){0.670046}
\ECirc(21.8462,7.10851){0.53812}
\ECirc(22.0703,5.76905){0.603132}
\ECirc(23.6881,0.383903){1.19548}
\ECirc(23.3269,6.14045){0.616912}
\ECirc(25.7079,2.52202){1.12431}
\ECirc(25.7097,3.43202){1.5124}
\ECirc(-5.37364,15.4443){0.707105}
\ECirc(39.3622,1.82626){0.236819}
\ECirc(38.7003,0.610934){0.549332}
\ECirc(38.2738,0.587901){0.467806}
\ECirc(41.5302,6.18229){0.708011}
\ECirc(43.3259,7.12447){0.649274}
\ECirc(42.0914,8.54099){0.701198}
\ECirc(-2.98729,-26.25){0.706892}
\ECirc(-1.12892,-27.835){0.570621}
\ECirc(2.71442,-28.0448){0.835772}
\ECirc(-1.01898,-23.5097){0.355335}
\ECirc(-0.940451,-23.9627){0.329698}
\ECirc(4.03596,-25.0288){0.520844}
\ECirc(45.1701,30.9658){0.975145}
\ECirc(39.057,28.6267){0.340482}
\ECirc(38.8531,31.6048){0.623574}
\ECirc(40.4578,37.2754){0.483935}
\ECirc(42.8047,34.0335){0.585562}
\ECirc(-26.0923,70.3561){0.906045}
\ECirc(31.4127,-46.9036){0.690708}
\ECirc(27.7752,-41.5785){0.599439}
\ECirc(6.44029,2.83659){0.697001}
\ECirc(-1.62932,-2.51559){0.45715}
\ECirc(-7.27281,-26.5921){1.10412}
\ECirc(-8.46789,-36.1197){0.750713}
\ECirc(-7.36419,-37.0127){0.87746}
\ECirc(-6.93106,-37.0028){0.87746}
\ECirc(26.8138,47.1544){0.970079}
\ECirc(26.0047,51.04){0.676619}
\ECirc(26.0574,55.8785){0.994122}
\ECirc(28.0478,-32.3831){1.28304}
\ECirc(21.115,-38.8834){0.40394}
\ECirc(17.8121,-40.378){0.652442}
\ECirc(18.3926,-39.9369){0.70597}
\ECirc(28.2353,-26.3017){0.799382}
\ECirc(27.1248,-26.0508){0.577188}
\ECirc(31.5004,-26.9029){0.396134}
\ECirc(29.8823,-25.3674){0.603083}
\ECirc(-18.9736,-8.63187){0.315971}
\ECirc(-16.767,-10.3894){0.431348}
\ECirc(-16.597,-13.7414){0.313781}
\ECirc(-16.817,-13.349){0.311812}
\ECirc(-14.0313,-11.9891){0.655221}
\ECirc(3.99885,-21.6241){1.03477}
\ECirc(5.00244,-26.9652){0.671974}
\ECirc(7.3443,-26.3593){0.964541}
\ECirc(7.21853,-23.4567){0.453988}
\ECirc(-21.3005,-14.4807){1.11443}
\ECirc(32.9101,28.5202){0.700833}
\ECirc(33.4535,26.1731){0.333679}
\ECirc(33.3018,27.6189){0.703581}
\ECirc(30.9655,30.4929){0.707023}
\ECirc(8.90407,-13.7645){0.707104}
\ECirc(-37.3328,45.9946){0.67445}
\ECirc(-25.2421,46.9759){0.707088}
\ECirc(-35.827,-36.3147){0.279435}
\ECirc(-36.7112,-40.1095){0.436697}
\ECirc(20.2824,-25.4753){1.2636}
\ECirc(-41.08,-5.90872){0.446804}
\ECirc(22.3911,-10.1668){0.695792}
\ECirc(44.4518,-0.246546){0.70709}
\ECirc(36.1927,0.463923){0.499419}
\ECirc(2.13322,11.4749){0.729881}
\ECirc(0.993675,15.0963){0.707083}
\ECirc(42.3282,21.5952){0.775133}
\ECirc(-31.9658,-34.5798){0.530355}
\ECirc(-6.86575,32.6503){0.739007}
\ECirc(-60.221,18.8444){1.12598}
\ECirc(-23.2463,1.77089){0.74989}
\ECirc(-22.6368,57.2645){0.484175}
\ECirc(-20.5809,51.4136){0.707038}
\ECirc(12.2744,-2.07726){0.387949}
\ECirc(38.6068,-1.86635){0.699884}
\ECirc(-26.1374,5.78808){0.415043}
\ECirc(-25.6494,7.17035){0.546753}
\ECirc(-48.8218,-22.192){0.706815}
\ECirc(26.5374,-13.4812){0.275913}
\ECirc(18.146,-22.1597){0.286329}
\ECirc(17.422,-22.4793){0.29837}
\ECirc(16.6158,-20.644){0.557262}
\ECirc(17.8226,-19.031){0.512325}
\ECirc(12.3884,-34.5018){0.707102}
\ECirc(-5.31785,47.0707){0.489641}
\ECirc(-38.205,-36.919){0.707104}
\ECirc(-31.3348,-35.4567){0.674588}
\ECirc(-50.8698,43.2111){0.494757}
\ECirc(0.220821,-45.5081){0.648954}
\ECirc(-1.03241,-45.116){0.667879}
\ECirc(2.37414,-45.0482){0.501971}
\ECirc(-27.9649,33.1186){0.704784}
\ECirc(-34.5476,35.2822){0.706543}
\ECirc(45.336,28.5537){0.705442}
\ECirc(46.3363,23.6656){0.444165}
\ECirc(43.4298,27.5864){0.803691}
\ECirc(47.3807,25.4907){1.02715}
\ECirc(17.7624,-8.20135){0.707095}
\ECirc(8.97678,-21.3025){0.706974}
\ECirc(18.8478,-52.4778){0.707107}
\ECirc(-11.5663,-48.8429){0.574103}
\ECirc(-1.70458,-7.45391){1.38054}
\ECirc(-37.9401,-2.22173){0.707107}
\ECirc(10.6447,-13.731){2.29917}
\ECirc(7.75542,-9.1839){0.415008}
\ECirc(8.98552,-12.795){0.489745}
\ECirc(9.82546,-17.7196){0.322957}
\ECirc(69.6561,15.9644){0.707069}
\ECirc(47.1658,-46.6477){0.702227}
\ECirc(-19.8933,-23.9598){0.745982}
\ECirc(8.73848,19.8322){0.695385}
\ECirc(-32.9366,30.5476){1.22395}
\ECirc(-37.4814,42.942){0.658159}
\ECirc(65.0391,-17.2311){0.532679}
\ECirc(4.35939,-14.4695){0.705118}
\ECirc(3.00503,-11.1425){0.555653}
\ECirc(2.61358,-11.5918){0.568521}
\ECirc(-0.216424,-8.80734){0.669176}
\ECirc(-2.48521,-4.1179){0.995059}
\ECirc(6.88713,-11.6305){1.01498}
\ECirc(5.63106,-13.0381){1.12512}
\ECirc(-5.60536,-26.2221){0.523745}
\ECirc(-4.90057,-27.9337){0.706833}
\ECirc(-5.30501,-30.2599){1.29309}
\ECirc(-3.34535,-22.1294){0.432913}
\ECirc(-1.39316,-24.0128){0.270858}
\ECirc(-2.61063,-25.2238){0.537625}
\ECirc(-3.19916,-23.5894){0.700454}
\ECirc(26.9412,59.401){1.00311}
\ECirc(-18.5936,20.5129){0.703877}
\ECirc(-57.7086,14.9509){0.700965}
\ECirc(-57.7103,21.5974){0.780672}
\ECirc(-52.5998,16.1786){0.50626}
\ECirc(-52.166,15.536){0.551244}
\ECirc(-58.6996,20.0436){0.899403}
\ECirc(-7.74676,-35.5579){0.483949}
\ECirc(-3.73189,-52.6955){0.704942}
\ECirc(38.7012,-43.1791){0.682216}
\ECirc(29.3844,64.6132){0.829607}
\ECirc(9.45859,6.74119){0.996646}
\ECirc(21.4758,33.6227){0.385503}
\ECirc(21.9444,28.7371){0.587897}
\ECirc(25.3741,17.2038){0.553886}
\ECirc(-18.9921,23.1612){1.20579}
\ECirc(-20.9129,24.0899){1.20609}
\ECirc(-20.7741,23.8761){1.04881}
\ECirc(-18.6732,22.6089){1.09407}
\ECirc(-17.7704,21.4911){1.09407}
\ECirc(28.0534,43.7861){0.428183}
\ECirc(-48.546,25.7951){0.525398}
\ECirc(27.1959,-21.4089){0.70704}
\ECirc(29.918,-27.53){0.696484}
\ECirc(18.7207,5.51073){1.01167}
\ECirc(14.9686,3.36228){0.516694}
\ECirc(12.6712,8.49126){0.947161}
\ECirc(42.0725,-25.2919){0.62163}
\ECirc(43.4383,-24.126){1.24907}
\ECirc(43.5016,-25.5638){0.678548}
\ECirc(42.9129,-22.6477){0.707092}
\ECirc(42.6198,-21.2309){0.706773}
\ECirc(65.3903,17.71){1.13307}
\ECirc(-14.4381,-18.0232){0.821544}
\ECirc(-6.18347,-8.91877){0.865022}
\ECirc(-9.23832,-13.5039){1.33408}
\ECirc(-19.228,-10.8629){0.838609}
\ECirc(-61.5429,-18.9676){0.707106}
\ECirc(12.4633,-30.5448){0.521308}
\ECirc(12.5076,-29.683){0.669319}
\ECirc(11.6921,-29.2398){0.699748}
\ECirc(6.77103,-28.7923){0.686624}
\ECirc(59.4275,28.431){1.8505}
\ECirc(29.5665,10.5145){0.670114}
\ECirc(31.2222,13.4531){0.342726}
\ECirc(30.6052,14.3417){0.554445}
\ECirc(-65.24,16.2625){0.707105}
\ECirc(-11.0627,65.5587){0.489763}
\ECirc(-34.4782,-33.6473){0.386174}
\ECirc(20.2831,29.6103){2.01298}
\ECirc(-22.0557,73.3922){0.634014}
\ECirc(-51.1682,1.49053){0.614705}
\ECirc(-31.9923,-14.1205){0.707092}
\ECirc(-25.2229,-6.70731){1.94189}
\ECirc(-27.0161,-16.0549){0.373096}


==> figs/PbPb-3.tex <==
\ECirc(-8.62478,-9.62978){0.936766}
\ECirc(25.9376,29.9129){0.612132}
\ECirc(22.7097,-40.1808){2.06013}
\ECirc(17.0184,-38.2434){1.00111}
\ECirc(46.6253,-13.4175){1.87114}
\ECirc(23.8,-26.055){1.31516}
\ECirc(-22.0768,-9.01244){1.4312}
\ECirc(26.799,36.6847){1.55521}
\ECirc(-2.41789,47.6456){1.8045}
\ECirc(5.29362,-51.1624){2.11796}
\ECirc(4.22556,-50.0069){1.87944}
\ECirc(19.961,-22.0072){1.44324}
\ECirc(-21.3962,-23.7603){1.90122}
\ECirc(-29.319,-46.3503){1.48578}
\ECirc(-22.796,-42.2534){1.78902}
\ECirc(-58.7742,15.5366){1.86476}
\ECirc(0.281175,-67.0534){1.95348}
\ECirc(35.8179,48.9146){1.91148}
\ECirc(-32.8865,4.37467){1.84842}
\ECirc(-24.7267,-8.55589){1.77034}
\ECirc(-26.3751,21.4785){1.09726}
\ECirc(7.84949,-22.8479){0.594189}
\ECirc(9.8488,-3.12753){1.54962}
\ECirc(-14.1015,-27.0624){1.48488}
\ECirc(-9.78953,47.7531){2.08095}
\ECirc(5.85545,33.8256){1.04089}
\ECirc(6.64106,38.3616){2.1166}
\ECirc(14.2955,-48.8512){0.839418}
\ECirc(-33.9065,-14.2022){1.99535}
\ECirc(26.249,40.885){1.73277}
\ECirc(24.5578,34.7977){2.04269}
\ECirc(-37.4106,13.3034){1.81407}
\ECirc(-24.323,6.10764){1.96055}
\ECirc(26.6901,38.0828){1.10148}
\ECirc(-37.3439,-40.7368){2.10165}
\ECirc(39.8033,-2.10367){0.499891}
\ECirc(-23.8237,45.5574){2.06914}
\ECirc(4.8375,-52.7205){1.85667}
\ECirc(-36.6387,-2.73714){1.24292}
\ECirc(25.7415,-15.3851){1.78448}
\ECirc(22.586,-37.5757){1.38572}
\ECirc(7.18888,-49.0746){1.05712}
\ECirc(5.27875,-47.5242){1.42032}
\ECirc(-37.7728,-5.8185){0.883017}
\ECirc(-36.7232,-33.7981){1.25586}
\ECirc(14.5896,-46.7109){0.819623}
\ECirc(21.9711,29.7715){1.60276}
\ECirc(6.15372,56.9272){1.71423}
\ECirc(-7.06794,44.6274){0.729543}
\ECirc(-6.72042,42.963){1.10117}
\ECirc(-1.42116,42.5635){1.71395}
\ECirc(-21.9016,-10.7456){1.92963}
\ECirc(11.1301,-47.3079){1.77128}
\ECirc(9.31791,-51.0724){1.02756}
\ECirc(4.28453,-13.9671){2.09906}
\ECirc(27.1584,9.46268){1.74672}
\ECirc(-39.8247,15.9019){1.34109}
\ECirc(-4.28089,-21.2614){1.85397}
\ECirc(21.1576,-11.2368){1.96508}
\ECirc(-40.1616,32.0583){1.97718}
\ECirc(40.8256,-7.25803){0.527315}
\ECirc(49.902,-25.4492){1.7629}
\ECirc(-1.15802,0.518107){2.00729}
\ECirc(5.88593,-53.6497){1.05225}
\ECirc(4.85904,39.3573){1.80503}
\ECirc(5.27491,37.9081){1.62718}
\ECirc(-4.73939,-7.07966){2.03143}
\ECirc(-23.0811,-17.8983){0.445716}
\ECirc(5.60989,44.9465){1.41876}
\ECirc(-8.915,-36.8887){2.05163}
\ECirc(-51.396,9.4402){1.55154}
\ECirc(-0.481516,-22.5129){2.11669}
\ECirc(20.144,30.7363){2.01313}
\ECirc(-38.2405,42.3466){1.26228}
\ECirc(-38.1609,36.8346){1.5424}
\ECirc(20.6805,-40.0122){1.45969}
\ECirc(38.7667,33.9838){1.96911}
\ECirc(7.03074,-7.64863){1.02191}
\ECirc(-32.3078,-5.30516){2.11236}
\ECirc(-14.1453,7.08541){1.65344}
\ECirc(28.4034,35.8564){2.11232}
\ECirc(10.6196,-12.5733){1.014}
\ECirc(14.5343,-10.6459){1.34047}
\ECirc(-13.3264,-37.728){0.767942}
\ECirc(-11.6754,-2.27513){0.796158}
\ECirc(11.5096,5.82152){1.80346}
\ECirc(-36.0019,12.8506){1.77201}
\ECirc(-35.0969,15.2495){0.603789}
\ECirc(-31.4612,4.29199){1.35997}
\ECirc(-15.9481,-41.3077){1.9473}
\ECirc(-14.2136,-28.6173){1.30589}
\ECirc(19.064,-37.6852){1.7929}
\ECirc(42.5562,7.59733){2.1063}
\ECirc(17.7998,-1.98327){2.05191}
\ECirc(-20.6021,-10.6248){2.02443}
\ECirc(18.8421,5.12026){0.720176}
\ECirc(-43.0704,-4.4102){2.07697}
\ECirc(30.3085,19.211){2.07032}
\ECirc(-52.1669,-27.5681){2.07474}
\ECirc(-39.5613,-8.33597){2.1022}
\ECirc(-23.5841,-7.81143){0.809015}
\ECirc(8.97156,-49.7865){1.61097}
\ECirc(-20.8749,-22.2795){2.14656}
\ECirc(-1.40341,50.9752){1.96125}
\ECirc(-11.9985,-56.9388){2.14977}
\ECirc(27.8783,-9.47609){2.07608}
\ECirc(55.8922,-3.4391){2.10445}
\ECirc(57.4704,-4.7563){1.18732}
\ECirc(58.2724,-3.59829){1.3228}
\ECirc(-6.50045,8.33983){0.897991}
\ECirc(21.5019,-35.1305){1.46456}
\ECirc(-45.2224,5.34499){0.620047}
\ECirc(-3.16678,50.3252){1.95541}
\ECirc(7.83016,-30.8913){2.09413}
\ECirc(-61.2633,8.39726){1.94893}
\ECirc(-11.9112,49.4146){1.39929}
\ECirc(-12.9977,49.7026){1.5916}
\ECirc(-14.8083,-24.0848){2.11342}
\ECirc(21.0611,-23.1786){2.11084}
\ECirc(-22.9306,-7.96927){1.42087}
\ECirc(44.6717,-32.3873){2.12081}
\ECirc(-9.72282,-7.12237){1.90418}
\ECirc(8.70501,35.1415){2.0241}
\ECirc(8.45832,37.773){1.23715}
\ECirc(64.6295,-17.6388){1.88371}
\ECirc(-7.44222,14.8895){2.09468}
\ECirc(-1.97194,17.3295){1.96399}
\ECirc(-26.6635,42.4698){3.40819}
\ECirc(-22.7758,38.2155){1.10311}
\ECirc(-4.42312,12.3001){1.577}
\ECirc(-4.07346,11.2869){0.68331}
\ECirc(1.60165,7.92627){0.861461}
\ECirc(-38.2982,-10.2666){0.565867}
\ECirc(-56.9926,40.725){2.03119}
\ECirc(24.7248,30.3457){1.72118}
\ECirc(5.08847,-2.40687){0.748734}
\ECirc(0.580145,-5.83508){1.62636}
\ECirc(29.8541,23.4465){2.12007}
\ECirc(-18.4605,60.2083){0.840657}
\ECirc(2.95596,53.5685){2.05528}
\ECirc(-10.7911,-21.2493){1.94153}
\ECirc(-36.4568,-9.75928){1.80011}
\ECirc(-35.818,-9.02969){2.10601}
\ECirc(29.9484,-25.0796){2.06254}
\ECirc(-1.15643,-3.4043){2.10938}
\ECirc(-9.41762,-8.53441){2.04482}
\ECirc(27.1421,5.42463){2.11905}
\ECirc(14.9489,-8.57969){1.84179}
\ECirc(5.01544,-0.935428){1.46193}
\ECirc(6.17707,4.54391){0.532576}
\ECirc(2.50149,3.84511){1.58943}
\ECirc(3.92182,-8.79228){2.08914}
\ECirc(24.8266,46.8825){1.537}
\ECirc(41.7094,3.69935){2.10622}
\ECirc(26.7241,76.0639){1.30272}
\ECirc(5.44719,35.2941){2.07627}
\ECirc(8.8954,-5.06647){1.31132}
\ECirc(-26.9903,-4.71066){1.84677}
\ECirc(-28.3536,-3.66796){1.75093}
\ECirc(-24.917,-1.97208){0.81955}
\ECirc(-30.0743,-5.11848){2.18432}
\ECirc(-6.96033,42.6181){1.96744}
\ECirc(-11.5432,41.6656){2.14934}
\ECirc(-13.3093,2.94582){2.07737}
\ECirc(12.8517,-51.228){2.11832}
\ECirc(4.23359,-2.212){1.18397}
\ECirc(4.95131,-3.26678){2.05554}
\ECirc(49.1836,28.2735){2.08504}
\ECirc(-26.8503,26.5968){2.11706}
\ECirc(12.4735,-47.3846){0.644408}
\ECirc(-36.7702,-40.9623){1.91596}
\ECirc(18.0995,-7.12027){2.10987}
\ECirc(19.7354,26.0107){0.774623}
\ECirc(-12.9944,-17.4375){2.11305}
\ECirc(-42.7198,-11.7133){2.04819}
\ECirc(24.2419,4.64219){2.06291}
\ECirc(39.1515,-1.90339){1.72231}
\ECirc(36.6048,-24.8037){1.2548}
\ECirc(49.1479,-0.502261){2.11628}
\ECirc(11.2762,56.6673){0.826589}
\ECirc(63.4387,16.7564){1.99817}
\ECirc(56.8439,-4.24983){1.05666}
\ECirc(55.2875,-4.06312){1.69323}
\ECirc(-26.419,-17.1862){1.83516}
\ECirc(2.70919,-54.8197){2.03812}
\ECirc(-3.18423,-4.92483){1.72654}
\ECirc(-1.93026,-1.5004){1.94859}
\ECirc(-6.5164,34.2216){2.11599}
\ECirc(7.37628,-50.0301){2.0287}
\ECirc(63.2639,-16.7465){1.01037}
\ECirc(9.31594,28.7891){1.18387}
\ECirc(52.4377,14.178){1.28506}
\ECirc(57.9712,19.8113){1.58569}
\ECirc(51.8521,17.8708){2.11771}
\ECirc(26.8243,-11.6394){2.05641}
\ECirc(11.3195,40.6588){1.87256}
\ECirc(62.3136,-21.5509){2.12029}
\ECirc(-23.4506,-15.8398){1.42535}
\ECirc(41.3485,7.15934){1.87954}
\ECirc(-0.127268,50.5622){0.90496}
\ECirc(0.528216,-43.7562){2.07112}
\ECirc(8.08704,2.93998){2.11605}
\ECirc(-12.7314,-7.00279){2.04083}
\ECirc(-12.5822,-32.5885){0.498204}
\ECirc(-9.58369,-34.0049){0.475121}
\ECirc(-11.0445,-36.0457){0.833909}
\ECirc(-10.0043,-29.3965){0.893325}
\ECirc(-9.28976,-40.6915){0.92053}
\ECirc(-35.6888,45.7173){1.87703}
\ECirc(23.0943,0.840943){2.11582}
\ECirc(-32.8228,1.11499){1.14595}
\ECirc(-44.2342,-2.65308){0.595888}
\ECirc(46.524,30.5084){1.96172}
\ECirc(41.3594,29.5973){1.80547}
\ECirc(41.05,30.5114){3.7191}
\ECirc(19.6563,7.90032){1.63193}
\ECirc(-35.108,13.3749){1.15907}
\ECirc(-35.0248,20.6827){1.04316}
\ECirc(-35.0985,19.1158){0.66868}
\ECirc(-35.2584,17.5474){0.497729}
\ECirc(-8.85927,-28.7569){1.1888}
\ECirc(50.5204,35.2446){0.532118}
\ECirc(50.6366,36.0712){1.42176}
\ECirc(-48.7025,-9.32254){0.982512}
\ECirc(-45.8193,-5.68025){0.930459}
\ECirc(-26.0633,20.3032){1.91541}
\ECirc(-43.3959,-28.2153){1.81166}
\ECirc(-49.7344,-24.9509){2.10383}
\ECirc(42.9007,-36.8786){1.3597}
\ECirc(-41.9315,32.7167){1.16642}
\ECirc(-22.9255,-9.73178){1.24413}
\ECirc(-46.2644,-14.7094){2.08475}
\ECirc(16.509,-57.6362){0.805344}
\ECirc(15.4883,-54.2369){2.07147}
\ECirc(1.56983,15.2887){2.06725}
\ECirc(18.279,-45.9532){1.53094}
\ECirc(16.9019,-44.4221){1.13087}
\ECirc(21.253,59.3694){2.00063}
\ECirc(21.4136,60.7045){2.05117}
\ECirc(5.60018,6.26893){1.74182}
\ECirc(4.82525,11.3268){1.81914}
\ECirc(5.86833,-15.5149){2.11644}
\ECirc(-20.5935,16.5702){1.05761}
\ECirc(-3.2179,-13.2957){0.513424}
\ECirc(-2.64205,-17.89){1.01294}
\ECirc(-4.63164,-13.1738){1.80446}
\ECirc(25.6815,-16.3825){1.24367}
\ECirc(3.82697,12.7473){1.03835}
\ECirc(3.22138,-0.425441){2.10072}
\ECirc(-26.5337,46.4956){0.508729}
\ECirc(-47.0024,-13.4903){2.05268}
\ECirc(-33.757,-35.7249){0.853027}
\ECirc(3.24153,60.3994){1.76451}
\ECirc(11.7145,-45.6462){1.31252}
\ECirc(10.1293,-33.0601){1.46617}
\ECirc(7.9583,0.690897){2.12124}
\ECirc(62.936,-19.1213){2.08052}
\ECirc(-32.4597,-47.2856){1.89787}
\ECirc(-32.4791,-46.3539){1.48871}
\ECirc(48.4499,29.7428){1.95493}
\ECirc(44.7432,30.7311){0.810862}
\ECirc(49.31,-39.4641){1.94756}
\ECirc(50.2988,-35.6482){1.60487}
\ECirc(1.45513,12.2548){1.74414}
\ECirc(-47.6662,-11.8321){2.1202}
\ECirc(16.0311,-32.4881){2.09509}
\ECirc(18.0755,-34.0517){1.58434}
\ECirc(19.0984,-31.348){1.928}
\ECirc(-12.2816,-21.7392){2.11372}
\ECirc(28.2725,32.0402){2.12057}
\ECirc(-15.1719,0.33927){1.34118}
\ECirc(-41.7398,1.82035){1.84195}
\ECirc(58.5535,-3.19354){2.11885}
\ECirc(38.201,-1.57517){1.91686}
\ECirc(38.4004,-1.79009){1.77349}
\ECirc(18.4963,-12.7659){2.10709}
\ECirc(-36.0354,-5.953){2.12019}
\ECirc(13.161,-4.30825){2.10615}
\ECirc(-34.7749,18.6352){1.82552}
\ECirc(-32.5656,19.0414){0.726733}
\ECirc(34.5361,-47.4856){1.97342}
\ECirc(-10.3474,10.2336){1.17449}
\ECirc(-10.7487,9.17645){1.11177}
\ECirc(-9.36561,7.26619){0.240694}
\ECirc(-17.4568,-19.7936){1.79915}
\ECirc(-37.1919,14.3133){1.21951}
\ECirc(-33.6128,9.95403){1.46759}
\ECirc(28.1689,28.2269){1.07969}
\ECirc(4.85545,1.80501){2.14589}
\ECirc(-18.8807,-24.0496){1.36236}
\ECirc(9.61792,3.6413){2.08549}
\ECirc(25.1872,31.7222){2.23743}
\ECirc(1.76825,54.6391){1.7704}
\ECirc(-34.0721,3.46263){0.915825}
\ECirc(-33.8176,4.53422){0.715863}
\ECirc(2.02935,50.8936){1.58746}
\ECirc(-21.1675,-15.8144){2.02266}
\ECirc(37.087,-3.11036){1.60178}
\ECirc(36.6697,2.28025){0.486516}
\ECirc(-5.1489,46.4214){2.10645}
\ECirc(21.7381,21.796){0.353134}
\ECirc(22.3004,18.2378){0.358617}
\ECirc(21.7987,23.9398){2.11714}
\ECirc(28.8996,24.1211){0.924273}
\ECirc(55.0887,36.7731){0.486426}
\ECirc(-16.2528,-20.135){1.27181}
\ECirc(-23.1927,-18.876){1.19809}
\ECirc(-17.258,2.85852){2.13031}
\ECirc(25.6105,-5.97216){2.04702}
\ECirc(22.0764,-21.604){2.09757}
\ECirc(-52.2358,2.17504){0.907005}
\ECirc(-47.7897,3.98238){0.956643}
\ECirc(5.93948,-2.46667){1.10142}
\ECirc(11.9199,0.0929624){1.68215}
\ECirc(21.2524,-38.3284){2.11969}
\ECirc(8.1919,33.1373){0.996066}
\ECirc(6.48982,35.1091){1.03119}
\ECirc(-17.3271,13.1327){1.58445}
\ECirc(-28.6545,-22.4649){1.79967}
\ECirc(46.5052,-8.04731){1.43058}
\ECirc(44.7859,-8.56019){1.40713}
\ECirc(44.3779,-8.21097){1.68268}
\ECirc(46.5409,-10.1197){2.03966}
\ECirc(-40.0878,-29.3259){2.02235}
\ECirc(-41.0893,-29.9719){1.71815}
\ECirc(-7.63978,-8.99608){0.828193}
\ECirc(20.1728,33.7574){1.73841}
\ECirc(19.9991,-37.7771){1.91977}
\ECirc(25.876,-38.6276){2.02612}
\ECirc(28.7479,-35.8933){1.9691}
\ECirc(33.0481,30.603){1.16779}
\ECirc(-8.28955,-0.0828806){2.07641}
\ECirc(13.796,-18.2714){1.93697}
\ECirc(-26.7798,48.614){1.23839}
\ECirc(-28.9492,46.9439){1.65667}
\ECirc(-15.8041,-10.6298){0.738413}
\ECirc(7.54536,0.905185){2.04867}
\ECirc(27.2831,20.7296){2.04575}
\ECirc(-3.11472,-4.32951){1.46129}
\ECirc(49.435,-13.1706){2.31212}
\ECirc(3.76915,-23.0122){1.05674}
\ECirc(4.49053,-29.4656){1.90981}
\ECirc(-9.11525,6.57785){1.75415}
\ECirc(15.6673,-50.8069){1.55346}
\ECirc(11.9833,-50.2448){1.64212}
\ECirc(11.3419,-49.9881){1.64296}
\ECirc(18.5503,-19.2569){1.94276}
\ECirc(22.7869,-26.168){0.52672}
\ECirc(-44.4025,1.83419){2.12052}
\ECirc(10.9561,-25.2937){1.08065}
\ECirc(3.41841,-28.1282){2.10739}
\ECirc(4.57639,-24.8344){0.917438}
\ECirc(11.2742,-28.4287){1.24426}
\ECirc(12.201,-2.35607){2.11557}
\ECirc(34.5007,-46.9912){1.91975}
\ECirc(30.9163,-42.7725){1.85834}
\ECirc(-8.00942,-37.6415){2.1173}
\ECirc(2.8034,15.9002){0.801876}
\ECirc(12.4187,-27.2734){2.11643}
\ECirc(11.9745,-24.9314){1.81875}
\ECirc(17.727,-24.3186){1.79656}
\ECirc(15.6578,-20.1008){0.933508}
\ECirc(-5.88618,-58.0654){2.12087}
\ECirc(41.0559,2.98794){2.10673}
\ECirc(41.9693,2.80463){1.54905}
\ECirc(44.2324,2.96992){1.03414}
\ECirc(-33.0011,-26.6144){1.89419}
\ECirc(4.41392,-13.634){2.1183}
\ECirc(15.929,-55.8655){1.96219}
\ECirc(-2.34009,25.3992){1.92064}
\ECirc(-36.8692,0.486937){0.939789}
\ECirc(18.299,-9.07091){1.48846}
\ECirc(15.3795,-7.8248){4.73904}
\ECirc(19.6923,-14.6657){0.665123}
\ECirc(33.1218,29.7176){2.1049}
\ECirc(33.4615,30.3568){2.10828}
\ECirc(46.7641,-10.7932){2.11954}
\ECirc(-11.9036,45.2241){2.10029}
\ECirc(-11.2796,-29.4411){1.19624}
\ECirc(0.214872,-4.62552){2.0637}
\ECirc(3.70365,-4.14482){2.111}
\ECirc(58.2828,-7.31434){0.750616}
\ECirc(-14.2497,-55.8085){2.09395}
\ECirc(-43.6134,39.1023){2.1095}
\ECirc(-48.7893,37.566){1.75293}
\ECirc(-48.7505,38.5541){1.65973}
\ECirc(-47.7645,32.8978){2.0672}
\ECirc(-7.22463,-4.00905){1.12421}
\ECirc(28.3077,29.4745){2.05807}
\ECirc(34.3531,-40.6455){1.89449}
\ECirc(42.1701,-44.2365){1.82267}
\ECirc(43.5622,-43.1275){1.86777}
\ECirc(1.47865,25.8481){2.1149}
\ECirc(-6.8766,-36.2535){2.11973}
\ECirc(15.4975,-3.31289){2.08392}
\ECirc(-15.0745,-35.8584){2.11521}
\ECirc(28.994,20.3674){2.1198}
\ECirc(54.3779,-0.131804){0.56927}
\ECirc(56.8857,1.55014){1.05404}
\ECirc(58.2993,3.43077){0.654427}
\ECirc(9.09719,8.57021){0.787538}
\ECirc(-20.3904,-18.6084){2.12048}
\ECirc(-3.4079,7.40066){2.05711}
\ECirc(-1.71921,0.120628){2.11941}
\ECirc(58.7925,-12.4569){1.93719}
\ECirc(-21.8334,6.45527){0.191184}
\ECirc(-20.9946,5.7478){0.941613}
\ECirc(-38.7045,-31.6435){1.96881}
\ECirc(-29.4383,-5.49738){3.5867}
\ECirc(18.1942,-5.12749){1.6232}
\ECirc(54.9158,43.7706){2.10735}
\ECirc(52.0241,43.8892){1.83008}
\ECirc(7.30973,-15.252){2.08952}
\ECirc(-46.7822,10.4186){1.15766}
\ECirc(-37.029,39.3209){0.898761}
\ECirc(-40.4412,1.06467){2.06952}
\ECirc(-41.4733,0.563617){1.7522}
\ECirc(50.2324,43.8552){2.10968}
\ECirc(-31.7634,27.7988){1.22113}
\ECirc(3.79235,-2.32768){2.13337}
\ECirc(12.1998,2.56225){2.11935}
\ECirc(13.3474,5.53983){2.07799}
\ECirc(20.3665,14.8492){0.980303}
\ECirc(-6.78697,-37.9805){2.08719}
\ECirc(-11.1201,-11.6606){1.20371}
\ECirc(-6.16888,-16.1032){2.01691}
\ECirc(-43.0957,-16.1631){2.11027}
\ECirc(-27.5533,-29.8417){1.68979}
\ECirc(-2.54962,-18.7934){2.08774}
\ECirc(-31.439,-19.9246){2.06102}
\ECirc(53.6076,14.1109){2.08609}
\ECirc(-13.5469,-56.035){2.0455}
\ECirc(-19.5233,56.0254){0.923298}
\ECirc(0.33401,-19.1964){0.897487}
\ECirc(-3.95304,-5.85229){2.1194}
\ECirc(-13.9164,-3.48867){2.04423}
\ECirc(-8.02124,-4.95968){2.01873}
\ECirc(44.9408,29.7109){2.07587}
\ECirc(-14.5317,-54.0184){2.09617}
\ECirc(25.0118,35.3793){2.12074}
\ECirc(44.8603,-16.1464){1.46133}
\ECirc(45.1444,-11.6055){0.577713}
\ECirc(49.4911,-14.0682){0.710498}
\ECirc(45.5,-18.7287){0.752008}
\ECirc(46.5911,-8.74712){1.80855}
\ECirc(51.6207,-9.50683){1.13501}
\ECirc(52.6275,-14.5967){1.94762}
\ECirc(50.8433,-14.8114){1.6603}
\ECirc(10.8054,-2.81297){2.11075}
\ECirc(10.4533,7.29809){0.745861}
\ECirc(-53.4374,33.4169){2.12095}
\ECirc(-12.6064,3.53103){1.95321}
\ECirc(-43.3259,7.15971){2.1207}
\ECirc(19.7438,28.907){1.04307}
\ECirc(23.998,34.8946){1.88084}
\ECirc(17.4377,35.8276){1.61782}
\ECirc(22.7588,38.0405){1.53502}
\ECirc(-54.7961,-19.0685){0.642349}
\ECirc(-54.0824,-22.4569){1.24147}
\ECirc(-46.1254,-16.8833){0.520922}
\ECirc(-11.8944,-20.1605){2.08802}
\ECirc(21.2666,-37.9373){2.00214}
\ECirc(42.6379,-3.26902){2.04412}
\ECirc(6.30553,-47.1378){2.1212}
\ECirc(7.5882,-56.8748){1.82003}
\ECirc(-57.999,20.4832){2.22795}
\ECirc(-57.9951,19.1549){0.701928}
\ECirc(-11.2044,6.89562){2.11086}
\ECirc(-1.75225,16.4439){1.83464}
\ECirc(1.92843,15.0131){2.08984}
\ECirc(-9.94192,48.0647){1.86851}
\ECirc(-9.24132,46.9142){0.922389}
\ECirc(-26.0947,35.2618){2.06518}
\ECirc(-27.5091,37.5941){0.960555}
\ECirc(23.5781,-38.0243){1.0653}
\ECirc(-16.8044,-43.8243){1.61574}
\ECirc(-8.71292,-43.7001){1.55028}
\ECirc(36.3496,39.8423){2.1087}
\ECirc(12.3946,-43.5602){2.108}
\ECirc(4.22751,-17.5312){2.11962}
\ECirc(39.7352,23.9402){1.57148}
\ECirc(-11.9717,-21.6439){2.12086}
\ECirc(-27.6,31.2666){1.56777}
\ECirc(-46.3345,-8.23523){2.12099}
\ECirc(-21.9864,19.536){0.461487}
\ECirc(-21.7643,24.3845){0.363201}
\ECirc(37.0595,-2.51022){2.09277}
\ECirc(38.5801,-4.6994){2.03475}
\ECirc(-45.6011,-26.2262){1.79802}
\ECirc(-35.615,43.9573){2.10293}
\ECirc(53.5178,35.1348){2.10951}
\ECirc(-56.8257,36.4387){2.11511}
\ECirc(61.4986,18.2734){2.10193}
\ECirc(51.6202,40.7706){2.11989}
\ECirc(17.5737,23.2113){2.12271}
\ECirc(14.588,-57.1453){2.1212}
\ECirc(-53.2802,3.12771){1.70689}
\ECirc(-2.38081,-1.274){2.15623}
\ECirc(0.907477,-0.767999){1.84771}
\ECirc(2.63667,2.2366){1.85614}
\ECirc(-6.53425,24.2123){1.96109}
\ECirc(-5.80483,31.1493){1.61142}
\ECirc(22.0124,-11.9614){2.11918}
\ECirc(-22.351,19.0481){2.11757}
\ECirc(-21.8136,5.74825){1.95218}
\ECirc(16.8837,29.0608){1.32229}
\ECirc(15.4466,26.6027){2.09515}
\ECirc(-18.3595,-16.1408){2.12113}
\ECirc(-25.7272,5.20401){2.03934}
\ECirc(-19.4799,18.8327){2.17064}
\ECirc(49.7951,-17.0931){1.97113}
\ECirc(31.2015,-28.6659){1.95929}
\ECirc(-12.1802,-39.9464){2.12102}
\ECirc(-39.5823,17.1548){1.97685}
\ECirc(30.525,9.09194){1.69995}
\ECirc(-18.5624,-50.6227){2.03183}
\ECirc(-19.4736,10.414){2.08803}
\ECirc(-27.0381,2.29134){1.46968}
\ECirc(-23.3887,5.93785){2.11705}
\ECirc(-28.7414,5.27089){1.34377}
\ECirc(4.90999,-22.7195){1.51956}
\ECirc(-28.1498,-6.86724){0.690848}
\ECirc(53.9906,-10.0923){2.11412}
\ECirc(-10.8853,-4.86705){2.09108}
\ECirc(-48.4799,6.54346){5}
\ECirc(-3.21006,44.4918){2.11794}
\ECirc(-24.2982,16.2916){0.50078}
\ECirc(-21.3769,21.8854){2.12078}
\ECirc(-10.6834,-38.5032){2.11424}
\ECirc(1.68564,-2.28668){2.12119}
\ECirc(14.0027,5.40842){1.88366}
\ECirc(14.3897,7.37323){0.483303}
\ECirc(14.573,7.62285){0.422008}
\ECirc(12.9542,3.56257){1.97536}
\ECirc(-21.5892,-6.00894){2.28018}
\ECirc(-38.5798,43.5529){1.01334}
\ECirc(-40.3408,45.5701){1.10681}
\ECirc(-33.4399,43.7839){1.09971}
\ECirc(22.7141,14.2623){2.10634}
\ECirc(28.0014,12.9325){1.35954}
\ECirc(36.6531,-38.2831){2.25133}
\ECirc(-49.7471,39.0102){1.26254}
\ECirc(18.4106,-35.1029){2.1162}
\ECirc(41.1902,9.05993){1.57947}
\ECirc(42.7852,10.1157){1.76797}
\ECirc(43.9874,8.30869){2.06986}
\ECirc(46.1841,-0.2653){1.99955}
\ECirc(-8.82175,-5.48438){2.12751}
\ECirc(-35.2937,-14.5256){2.12131}
\ECirc(36.3375,-30.0164){2.12122}
\ECirc(-65.5669,6.99442){1.4706}
\ECirc(-52.6406,30.7601){1.71565}
\ECirc(-49.807,33.1577){1.91106}
\ECirc(-48.3484,36.112){1.82647}
\ECirc(-53.5205,22.5588){1.48042}
\ECirc(-55.9011,19.4389){1.94297}
\ECirc(17.9915,-39.2001){2.12069}
\ECirc(-22.8153,45.7498){0.918052}
\ECirc(-30.6262,43.7523){0.892557}
\ECirc(-31.9064,45.4429){0.848534}
\ECirc(46.2292,-35.0626){1.16282}
\ECirc(46.372,-35.9965){0.497137}
\ECirc(46.3662,-34.3581){0.627568}
\ECirc(49.9335,-37.7968){1.75387}
\ECirc(3.91034,-11.7523){1.56213}
\ECirc(4.24568,-10.7962){2.00225}
\ECirc(5.08153,-9.36135){2.07259}
\ECirc(8.36808,-11.2011){1.66757}
\ECirc(7.34341,-12.3829){1.87567}
\ECirc(8.59405,-5.74534){1.75068}
\ECirc(16.5695,-13.0838){1.05826}
\ECirc(19.9927,-13.325){1.18272}
\ECirc(51.6298,-28.7588){2.11112}
\ECirc(47.9227,-32.1978){0.959077}
\ECirc(47.887,-32.3003){0.754161}
\ECirc(49.4969,-32.8127){0.636162}
\ECirc(6.67438,7.19019){2.05097}
\ECirc(9.18476,0.212616){2.08785}
\ECirc(-31.0625,-17.8947){2.12124}
\ECirc(-17.2543,-47.0029){1.0574}
\ECirc(-13.9509,-44.0182){1.15883}
\ECirc(-12.1736,-45.2488){0.765683}
\ECirc(-15.7243,-44.2523){1.20328}
\ECirc(23.991,-24.2457){2.02677}
\ECirc(-28.7707,20.9061){2.15699}
\ECirc(-9.06033,-22.2409){1.83397}
\ECirc(-28.2521,30.4228){2.10586}
\ECirc(16.6798,-32.9573){2.1128}
\ECirc(6.38824,-31.042){1.29592}
\ECirc(7.18598,-30.1293){2.11023}
\ECirc(-20.3873,12.7092){2.11063}
\ECirc(-21.9593,12.2462){1.38014}
\ECirc(-57.0508,-28.4607){2.09988}
\ECirc(12.0656,-35.7813){2.12054}
\ECirc(31.1525,36.4687){1.99302}
\ECirc(10.5243,-49.1727){2.11711}
\ECirc(15.2098,-49.7147){2.12026}
\ECirc(-24.8047,30.7028){2.02256}
\ECirc(-30.6523,35.4785){2.10763}
\ECirc(-30.1461,34.5051){1.47473}
\ECirc(-31.9308,32.2305){0.999737}
\ECirc(23.3633,67.2245){1.65495}
\ECirc(22.1873,68.3626){1.10936}
\ECirc(21.0908,68.7702){1.39513}
\ECirc(20.9868,-42.1047){2.12124}
\ECirc(-16.7498,-11.6608){2.12053}
\ECirc(27.3175,30.3898){1.99687}
\ECirc(55.5481,39.4206){0.531276}
\ECirc(38.3174,27.9104){2.11721}
\ECirc(45.6697,29.5891){1.284}
\ECirc(48.2397,-25.2406){1.96934}
\ECirc(20.1558,30.585){2.12087}
\ECirc(22.8076,30.7501){0.883017}
\ECirc(-7.51811,9.11701){0.62661}
\ECirc(-7.9007,8.33457){0.61498}
\ECirc(-8.20481,10.8413){0.937098}
\ECirc(11.2229,-26.9233){2.0996}
\ECirc(10.7756,-22.6449){1.54784}
\ECirc(8.80345,-24.9493){0.696862}
\ECirc(8.71738,-25.3562){0.723499}
\ECirc(-25.8383,-21.8624){2.12124}
\ECirc(8.88901,-62.1692){2.12053}
\ECirc(11.6803,0.133882){0.957355}
\ECirc(19.2786,-26.9388){1.58905}
\ECirc(21.7117,-28.3958){0.944809}
\ECirc(54.4545,38.8993){0.704552}
\ECirc(53.1737,35.1463){2.10909}
\ECirc(31.0937,10.4837){1.9307}
\ECirc(-35.165,15.1544){0.982527}
\ECirc(41.8048,10.408){1.96903}
\ECirc(37.3568,13.3701){0.922872}
\ECirc(38.6706,14.0184){0.968641}
\ECirc(-16.2271,-28.919){2.02657}
\ECirc(-15.9515,-29.4883){2.10123}
\ECirc(-44.792,-10.4425){2.11963}
\ECirc(7.59572,-33.5745){2.12123}
\ECirc(-6.17756,-12.6173){2.11993}
\ECirc(-11.2374,-6.35211){0.657527}
\ECirc(-8.20021,-1.12177){1.64704}
\ECirc(-6.70414,-4.78243){2.03505}
\ECirc(-13.7456,-1.35453){1.46711}
\ECirc(-10.1388,-37.2103){1.87515}
\ECirc(-11.1347,-38.2842){1.9922}
\ECirc(43.5281,-10.1424){2.1204}
\ECirc(45.5705,-11.1669){1.86802}
\ECirc(-9.14681,-2.214){0.797781}
\ECirc(-36.3309,4.26167){2.13087}
\ECirc(-37.2426,2.28777){0.942816}
\ECirc(-42.0657,-3.35699){1.83038}
\ECirc(-16.9541,23.2868){2.11901}
\ECirc(-14.9478,23.0195){1.39773}
\ECirc(-52.6524,29.6876){1.86963}
\ECirc(-54.134,31.6121){2.11138}
\ECirc(63.9201,-19.663){1.37134}
\ECirc(-24.4302,-4.23898){2.07787}
\ECirc(-16.0598,-9.85161){1.23838}
\ECirc(-19.8491,-5.07687){1.2562}
\ECirc(-19.747,-3.42338){0.642005}
\ECirc(25.4579,-40.1351){1.26223}
\ECirc(22.5885,-42.3104){0.730921}
\ECirc(21.169,-42.7118){0.545559}
\ECirc(-47.6861,38.1673){2.12029}
\ECirc(-11.967,11.7426){0.920783}
\ECirc(-33.3375,10.8247){1.20163}
\ECirc(41.786,-34.5848){2.11198}
\ECirc(53.6798,-31.1845){1.49805}
\ECirc(8.0567,-46.0119){2.09806}
\ECirc(-20.0859,-6.20657){1.91397}
\ECirc(-19.9297,-8.59248){1.11563}
\ECirc(-18.7031,-13.3671){0.771601}
\ECirc(-19.0683,-11.0236){0.602185}
\ECirc(-14.5959,-16.0061){2.12021}
\ECirc(61.6367,-10.4058){2.11984}
\ECirc(-36.8135,-1.46835){0.503874}
\ECirc(6.84568,-0.488297){2.1341}
\ECirc(-16.4628,-33.1548){2.12127}
\ECirc(6.55477,36.257){2.12111}
\ECirc(4.30021,37.8099){1.39759}
\ECirc(67.9596,-20.2297){2.12002}
\ECirc(-53.383,8.42759){2.10369}
\ECirc(-19.42,-19.0515){2.11965}
\ECirc(11.4756,-50.9363){2.09692}
\ECirc(9.01216,-49.793){1.58194}
\ECirc(19.3542,-55.7983){2.12122}
\ECirc(-39.9329,42.7563){1.78253}
\ECirc(-36.4883,41.2062){1.74202}
\ECirc(44.0677,37.115){0.862951}
\ECirc(-34.1131,13.4613){1.73094}
\ECirc(-49.213,34.5161){1.05858}
\ECirc(-6.18659,-38.8571){2.06132}
\ECirc(-6.12817,-34.525){0.991764}
\ECirc(-6.60803,-39.3538){0.921641}
\ECirc(-1.07286,-1.06034){2.11113}
\ECirc(-59.9863,14.3257){2.12451}
\ECirc(50.2549,-33.7678){0.818335}
\ECirc(47.7089,-37.7919){0.565447}
\ECirc(45.0228,-33.8694){0.936505}
\ECirc(-15.1719,1.52442){2.11267}
\ECirc(30.861,-40.3932){2.11919}
\ECirc(29.2181,-42.633){1.42781}
\ECirc(28.2519,-41.5476){1.5823}
\ECirc(-31.0812,12.9264){0.694102}
\ECirc(-57.0273,18.7403){2.12075}
\ECirc(46.6672,36.4181){2.12076}
\ECirc(43.1412,30.7624){1.98337}
\ECirc(17.9958,42.9616){2.1261}
\ECirc(9.36028,-47.9953){2.12128}
\ECirc(-50.6632,8.33546){1.67011}
\ECirc(-49.5536,25.9593){0.721892}
\ECirc(-54.439,23.8392){0.723005}
\ECirc(-49.9754,21.9198){0.922103}
\ECirc(-49.0178,20.36){1.50758}
\ECirc(-8.79758,-23.4654){2.12127}
\ECirc(9.73464,-53.5325){0.879807}
\ECirc(-37.781,-11.6695){1.04618}
\ECirc(-39.0682,-8.28376){2.12073}
\ECirc(-54.1871,25.7624){2.12129}
\ECirc(-14.0133,-51.6255){2.12066}
\ECirc(6.46928,-38.1781){2.11015}
\ECirc(-22.7795,18.6562){2.12098}
\ECirc(-31.3936,-29.506){1.10517}
\ECirc(-26.4936,-33.157){1.71295}
\ECirc(-32.2351,-19.6995){1.24122}
\ECirc(4.65496,-13.4556){1.09387}
\ECirc(3.03785,-31.9095){0.895515}
\ECirc(-11.8635,28.0248){2.07597}
\ECirc(-13.3765,29.837){2.11681}
\ECirc(-48.8022,26.8397){1.85039}
\ECirc(6.3068,8.71239){2.10786}
\ECirc(8.37105,-49.1605){2.02723}
\ECirc(-31.3889,4.2895){2.12128}
\ECirc(20.2156,-18.9555){0.652288}
\ECirc(21.5281,-8.04472){1.14575}
\ECirc(24.74,-10.1416){1.28501}
\ECirc(-6.59639,-17.1342){2.1213}
\ECirc(0.829703,3.53402){2.14708}
\ECirc(9.56197,3.16378){2.12142}
\ECirc(16.7978,27.0334){0.754735}
\ECirc(2.06512,29.635){2.12684}
\ECirc(-12.6161,39.314){2.11904}
\ECirc(-19.4441,42.1241){1.15111}
\ECirc(-7.78873,39.6367){1.69309}
\ECirc(43.1335,-38.3004){0.755406}
\ECirc(-10.793,-7.12801){2.12129}
\ECirc(-55.8924,16.5771){2.12403}
\ECirc(-33.8894,-6.51057){2.1182}
\ECirc(5.23049,25.8632){2.11883}
\ECirc(47.0745,-51.6026){1.70707}
\ECirc(-7.72405,24.9468){2.12046}
\ECirc(47.6663,13.49){2.12047}
\ECirc(11.4143,-34.0784){0.587591}
\ECirc(6.88449,-33.7637){0.721313}
\ECirc(-8.33533,-50.8446){1.19657}
\ECirc(-6.18198,-49.4838){1.64077}
\ECirc(-6.3793,-48.8545){1.18783}
\ECirc(-8.28073,-50.8444){1.73079}
\ECirc(-5.10233,-50.9669){1.82335}
\ECirc(-3.4414,-53.3494){2.12122}
\ECirc(11.9759,-47.8689){1.05982}
\ECirc(12.1135,-49.4976){1.54897}
\ECirc(12.9349,-51.7468){1.97643}
\ECirc(14.4005,-50.5924){1.02083}
\ECirc(13.5179,-19.2435){2.12126}
\ECirc(-22.1687,-24.8204){2.12118}
\ECirc(-4.95798,1.58943){2.11557}
\ECirc(48.1743,29.9491){0.939029}
\ECirc(2.01923,52.9079){2.12065}
\ECirc(46.9954,-10.1039){2.12068}
\ECirc(21.2437,-0.378767){2.12222}
\ECirc(-45.0117,-8.73341){1.22263}
\ECirc(-45.3731,-11.2256){0.741765}
\ECirc(-46.192,-12.8892){0.652922}
\ECirc(-24.5895,32.5737){1.50905}
\ECirc(-24.8755,31.6852){1.49739}
\ECirc(-20.7763,41.5869){1.95408}
\ECirc(61.5549,-17.5467){2.12132}
\ECirc(3.50671,-3.66667){2.10973}
\ECirc(0.268254,17.7851){1.99315}
\ECirc(2.10057,17.7466){2.11623}
\ECirc(-39.623,-6.80554){2.11909}
\ECirc(41.5081,2.77128){2.11984}
\ECirc(26.8126,28.1124){1.5833}
\ECirc(-2.20258,-25.6003){2.1213}
\ECirc(21.1523,-10.8566){2.12099}
\ECirc(-1.96898,21.1821){1.59901}
\ECirc(-37.9754,1.75928){1.79669}
\ECirc(-39.4979,10.1984){0.987497}
\ECirc(9.77192,-6.10038){2.12128}
\ECirc(-6.23761,-9.63332){2.12123}
\ECirc(-17.9696,6.68152){1.45427}
\ECirc(-15.4377,-11.8287){2.12131}
\ECirc(26.6707,-12.7038){2.12114}
\ECirc(-22.1636,-21.9294){1.94797}
\ECirc(-35.3709,-35.3144){2.12032}
\ECirc(-30.1335,36.3178){2.12123}
\ECirc(18.1272,-9.01319){0.68589}
\ECirc(16.9396,-8.44745){1.77434}
\ECirc(28.1418,-11.828){0.373883}
\ECirc(26.6949,-13.2443){1.08495}
\ECirc(27.1225,-9.8153){0.863735}
\ECirc(8.55041,-21.5288){1.30273}
\ECirc(9.3519,-26.2048){1.37977}
\ECirc(11.786,-24.7448){0.792079}
\ECirc(9.11494,-26.0764){2.1202}
\ECirc(8.70485,35.94){0.974316}
\ECirc(5.01846,32.8657){0.974316}
\ECirc(2.61224,35.4477){0.604449}
\ECirc(2.51668,35.8476){0.691208}
\ECirc(9.75068,-53.5138){2.12061}
\ECirc(10.7903,-21.2744){2.1213}
\ECirc(-27.8404,-11.8137){2.1211}
\ECirc(-0.483033,53.891){2.12167}
\ECirc(-1.59221,14.8114){1.27576}
\ECirc(-1.38005,17.536){2.38016}
\ECirc(-47.0002,25.4493){2.68533}
\ECirc(-47.348,23.0913){1.43074}
\ECirc(-44.9352,24.72){2.14128}
\ECirc(-44.7665,27.3748){0.800638}
\ECirc(-45.5196,27.4258){0.601333}
\ECirc(-16.6451,-9.89216){2.12125}
\ECirc(-21.3407,18.4013){1.2296}
\ECirc(-30.7188,15.513){0.836593}
\ECirc(-27.1811,17.5754){1.28975}
\ECirc(20.6524,-37.2575){0.556198}
\ECirc(5.21048,31.6969){2.11127}
\ECirc(3.78964,33.7534){0.489983}
\ECirc(3.99459,33.015){0.328953}
\ECirc(4.16868,32.5947){0.328953}
\ECirc(22.7098,23.5462){1.64719}
\ECirc(19.6564,24.1271){2.11996}
\ECirc(21.4945,32.9947){0.450283}
\ECirc(-40.5182,-30.7031){2.12107}
\ECirc(-39.5372,1.62714){0.663808}
\ECirc(-0.817396,2.21521){2.11599}
\ECirc(26.34,33.0991){0.990424}
\ECirc(24.3503,29.9514){0.75393}
\ECirc(-32.892,-15.0315){3.05063}
\ECirc(-5.11499,-15.8668){2.1576}
\ECirc(34.8568,-26.9832){1.99909}
\ECirc(-41.0528,-28.2519){1.71447}
\ECirc(-45.158,-20.8733){1.87801}
\ECirc(-0.628222,-13.8445){1.77809}
\ECirc(22.7542,44.3324){2.11995}
\ECirc(-33.9672,37.9368){2.11778}
\ECirc(16.2207,7.09912){2.2962}
\ECirc(54.8634,9.40237){1.52654}
\ECirc(58.6083,10.7822){1.2979}
\ECirc(53.9389,11.8683){1.08727}
\ECirc(-36.4187,30.9769){1.8579}
\ECirc(-27.8261,29.9635){2.12065}
\ECirc(-1.33936,54.1258){0.723786}
\ECirc(0.255149,55.1081){0.690225}
\ECirc(1.7436,55.5875){0.85918}
\ECirc(-1.64875,54.1376){0.381661}
\ECirc(-1.73077,54.3706){1.94173}
\ECirc(10.9493,-25.6096){2.12131}
\ECirc(42.6411,-12.783){1.82531}
\ECirc(14.4046,7.40064){2.12933}
\ECirc(-17.1651,6.75885){2.12124}
\ECirc(-7.53899,-3.59677){0.50175}
\ECirc(5.16912,33.783){2.10853}
\ECirc(31.7141,-23.3554){1.17869}
\ECirc(16.038,-35.9636){2.12671}
\ECirc(13.819,-49.246){2.12109}
\ECirc(43.9643,4.84734){2.10825}
\ECirc(42.2836,8.06869){1.89908}
\ECirc(-27.4697,49.7317){0.85506}
\ECirc(-27.0339,49.1953){1.11402}
\ECirc(4.76223,-1.00606){2.15138}
\ECirc(-11.1175,26.3088){1.74119}
\ECirc(-13.4463,24.9977){0.814906}
\ECirc(-16.2198,29.2939){0.887346}
\ECirc(-18.8681,23.6762){2.07595}
\ECirc(-8.91078,67.3213){1.90278}
\ECirc(7.15632,-58.9304){2.1212}
\ECirc(-10.2829,5.39085){1.19914}
\ECirc(1.90273,5.10329){2.13716}
\ECirc(-39.078,-8.16786){1.93977}
\ECirc(-45.186,-10.3961){0.821671}
\ECirc(-30.9328,-9.42759){0.949105}
\ECirc(28.242,11.8494){2.11703}
\ECirc(55.271,41.7509){2.12131}
\ECirc(59.7519,26.9269){2.03687}
\ECirc(53.4008,17.6149){2.05722}
\ECirc(-8.34735,47.2732){1.92586}
\ECirc(-10.2112,45.3759){1.28865}
\ECirc(-10.3349,45.6196){1.00721}
\ECirc(23.6895,-11.0816){2.12091}
\ECirc(-38.1901,-0.419184){1.14657}
\ECirc(1.79831,22.3404){2.11968}
\ECirc(2.32559,-15.1719){2.12131}
\ECirc(8.35179,-18.1128){1.49494}
\ECirc(8.09333,-9.80608){2.11734}
\ECirc(44.3495,-22.3969){2.04249}
\ECirc(56.7724,-10.0068){0.790647}
\ECirc(58.7533,-10.7072){0.551665}
\ECirc(57.0176,-11.5522){0.706653}
\ECirc(-15.199,-13.8683){2.12045}
\ECirc(-24.3984,51.2016){1.20401}
\ECirc(-22.1335,50.8034){1.77224}
\ECirc(-22.0286,53.3639){2.11774}
\ECirc(-4.24512,-60.678){2.06911}
\ECirc(-0.477938,-62.0247){1.72162}
\ECirc(1.86797,-58.7938){1.41622}
\ECirc(2.85623,-58.3148){0.733814}
\ECirc(-46.8469,-17.7344){1.23273}
\ECirc(-24.3804,32.9948){1.45963}
\ECirc(24.8657,45.4166){2.12132}
\ECirc(-10.9752,-23.1181){1.48324}
\ECirc(-44.0816,-14.196){2.11036}
\ECirc(-39.2957,-15.6547){2.11745}
\ECirc(10.9561,-25.1091){2.12132}
\ECirc(-39.5416,21.1396){2.11712}
\ECirc(-28.5735,33.236){0.525704}
\ECirc(-36.3091,28.4012){0.498029}
\ECirc(12.5497,23.8038){1.66978}
\ECirc(16.0529,21.4641){1.55588}
\ECirc(15.6901,21.8258){1.39748}
\ECirc(-1.38003,-18.3965){2.12105}
\ECirc(-2.38252,24.1577){1.21571}
\ECirc(-7.08608,28.6354){0.962467}
\ECirc(-6.15598,27.02){1.03278}
\ECirc(-41.9693,-14.3899){1.56693}
\ECirc(-41.0619,-7.57302){2.12127}
\ECirc(-42.4669,-9.2958){1.888}
\ECirc(-41.9682,-6.76729){1.31577}
\ECirc(-37.3441,-6.93705){0.499107}
\ECirc(-41.22,-5.52766){0.304419}
\ECirc(1.61434,-2.39826){1.16942}
\ECirc(-2.16165,11.1834){1.43577}
\ECirc(-2.54386,10.5526){0.575098}
\ECirc(-2.92638,13.673){0.646919}
\ECirc(-3.3874,16.1341){1.39771}
\ECirc(67.7917,-16.3201){2.07325}
\ECirc(3.6107,29.112){1.75234}
\ECirc(-12.6506,0.291694){2.12177}
\ECirc(-4.82425,-3.8789){2.10332}
\ECirc(-29.2106,45.9032){1.82005}
\ECirc(-27.371,38.7887){2.1196}
\ECirc(-1.81995,-57.4566){2.12123}
\ECirc(7.48427,-4.28593){2.1211}
\ECirc(-26.8987,46.7387){2.12115}
\ECirc(-24.5211,49.0966){1.43182}
\ECirc(-24.0313,46.408){1.55779}
\ECirc(-29.6144,44.3074){1.67358}
\ECirc(13.6649,-4.90954){2.121}
\ECirc(5.4769,-3.70126){0.690309}
\ECirc(7.6175,0.832381){1.85584}
\ECirc(-6.9365,30.5567){2.1043}
\ECirc(-8.58754,29.5851){1.27042}
\ECirc(-5.05419,34.2583){1.72744}
\ECirc(-14.0164,29.7809){2.06283}
\ECirc(-4.54516,34.2381){1.15416}
\ECirc(-6.80242,19.9411){2.11876}
\ECirc(-8.88019,18.5889){1.22339}
\ECirc(-39.3007,16.0036){2.10536}
\ECirc(-2.62184,16.3229){1.26208}
\ECirc(30.6706,46.2247){1.4387}
\ECirc(21.702,41.51){0.856984}
\ECirc(21.938,41.8493){1.37408}
\ECirc(21.5862,48.6298){1.33499}
\ECirc(22.412,-32.9848){1.51845}
\ECirc(-15.2664,-23.1176){1.32222}
\ECirc(-28.8032,-10.4547){1.46534}
\ECirc(-17.4412,-17.7339){1.72573}
\ECirc(-23.386,58.1531){2.12129}
\ECirc(-17.4729,-25.4064){2.1212}
\ECirc(38.9577,31.2287){0.705215}
\ECirc(38.199,33.7565){2.06835}
\ECirc(7.37759,-31.0462){1.01225}
\ECirc(8.8238,-19.6581){0.790377}
\ECirc(7.48443,-17.2726){1.60226}
\ECirc(8.73057,-17.8917){1.67294}
\ECirc(7.55219,-13.7999){2.12121}
\ECirc(59.6616,-4.58392){1.0142}
\ECirc(56.0332,-0.495585){2.12105}
\ECirc(17.8196,-18.7386){0.902995}
\ECirc(-30.3242,-8.72893){2.12128}
\ECirc(-26.0121,-21.8961){0.968535}
\ECirc(-11.4796,26.0991){1.63646}
\ECirc(-12.6549,23.8651){2.05214}
\ECirc(-49.1072,46.9218){0.524467}
\ECirc(-48.2962,45.5352){1.10268}
\ECirc(-34.5482,30.4028){2.12126}
\ECirc(-1.12593,-3.26438){1.46141}
\ECirc(1.55147,-0.536629){1.55538}
\ECirc(6.54622,0.420005){1.51793}
\ECirc(48.1279,16.851){2.12077}
\ECirc(-52.963,-19.4197){2.1212}
\ECirc(-30.0994,5.95524){1.87361}
\ECirc(-36.0998,4.51558){1.93461}
\ECirc(-39.2979,2.27908){0.788695}
\ECirc(-38.4801,0.904515){1.31114}
\ECirc(-9.19555,6.54376){0.690704}
\ECirc(-10.5429,2.17566){0.690704}
\ECirc(-11.271,3.39533){1.16907}
\ECirc(8.02088,7.76192){1.98986}
\ECirc(5.58493,38.5639){2.12124}
\ECirc(4.93189,36.1923){1.06835}
\ECirc(4.25898,35.8987){0.468923}
\ECirc(4.15321,37.3219){0.815475}
\ECirc(-18.6283,-37.8103){0.96972}
\ECirc(-19.1811,-37.7494){1.25988}
\ECirc(-22.736,-35.513){1.43241}
\ECirc(19.968,23.9738){1.18059}
\ECirc(-4.53508,-42.5943){2.08969}
\ECirc(-7.76842,-44.3833){0.898931}
\ECirc(-52.7519,23.1577){2.12097}
\ECirc(-23.6575,-25.2986){1.00119}
\ECirc(-27.4568,-25.1513){1.42472}
\ECirc(-33.586,-12.5213){1.9394}
\ECirc(43.7948,30.5592){0.456196}
\ECirc(20.8615,3.77022){2.01014}
\ECirc(23.6048,7.25218){0.998745}
\ECirc(22.8995,4.09784){0.764529}
\ECirc(23.7197,0.39657){2.12101}
\ECirc(25.3253,6.07099){0.616912}
\ECirc(27.7065,2.45256){1.12431}
\ECirc(25.778,4.07819){2.00625}
\ECirc(-5.37441,15.4396){2.12131}
\ECirc(37.9107,3.18223){0.247772}
\ECirc(38.9942,1.83546){1.648}
\ECirc(37.311,2.18792){0.759579}
\ECirc(41.5741,6.13161){2.12013}
\ECirc(42.918,6.44541){1.94782}
\ECirc(42.2033,8.3085){2.10359}
\ECirc(-3.0147,-26.2909){2.12068}
\ECirc(0.299462,-29.099){0.638217}
\ECirc(3.1574,-29.646){1.18104}
\ECirc(-2.12577,-25.1194){0.45479}
\ECirc(-2.52432,-24.919){0.805568}
\ECirc(4.32089,-23.1601){0.692909}
\ECirc(44.9111,29.0178){0.975145}
\ECirc(40.0456,26.9254){0.380075}
\ECirc(39.7725,31.8142){1.87072}
\ECirc(40.2105,39.0683){0.902706}
\ECirc(42.0862,34.8942){1.75669}
\ECirc(-26.0912,70.3602){2.12132}
\ECirc(31.2707,-47.3076){2.07212}
\ECirc(27.3882,-40.5908){1.79832}
\ECirc(6.1281,2.9633){2.091}
\ECirc(-1.9887,-3.99848){1.37145}
\ECirc(-7.27501,-26.5927){2.12132}
\ECirc(-8.02604,-37.8645){0.924855}
\ECirc(-6.86875,-38.8655){0.87746}
\ECirc(-6.1046,-38.5748){0.975536}
\ECirc(27.977,46.7815){1.67972}
\ECirc(26.4753,51.3806){2.02986}
\ECirc(25.9815,55.7243){2.11348}
\ECirc(28.9589,-32.2672){1.8844}
\ECirc(19.4288,-39.187){1.09429}
\ECirc(16.7954,-41.3152){1.53265}
\ECirc(18.292,-39.9891){2.11791}
\ECirc(28.2629,-26.308){2.12111}
\ECirc(26.5575,-25.0443){1.73156}
\ECirc(30.5233,-28.4785){0.795743}
\ECirc(31.1561,-23.872){0.603083}
\ECirc(-19.2699,-6.69849){0.442758}
\ECirc(-17.5351,-11.7756){1.29404}
\ECirc(-17.8895,-15.2251){0.379362}
\ECirc(-18.4889,-14.3158){0.551469}
\ECirc(-13.3246,-11.7319){1.96566}
\ECirc(4.80307,-21.818){1.93135}
\ECirc(4.42606,-26.7298){2.01592}
\ECirc(6.04105,-27.1267){1.38803}
\ECirc(6.91033,-24.9588){1.36196}
\ECirc(-21.3029,-14.4759){2.10739}
\ECirc(32.6637,28.4204){2.1025}
\ECirc(34.9281,25.1055){0.878508}
\ECirc(33.4418,27.761){2.11074}
\ECirc(30.935,30.4878){2.12107}
\ECirc(8.90874,-13.767){2.12131}
\ECirc(-37.01,47.6862){1.0814}
\ECirc(-25.2278,46.9783){2.12126}
\ECirc(-34.3421,-35.2329){0.838305}
\ECirc(-35.4696,-41.0754){1.31009}
\ECirc(19.1582,-24.1663){1.2636}
\ECirc(-42.6688,-4.74845){0.446804}
\ECirc(22.138,-9.91596){2.08738}
\ECirc(44.4383,-0.247973){2.12127}
\ECirc(37.5605,1.6946){0.83151}
\ECirc(2.15165,11.4787){2.12123}
\ECirc(1.0101,15.0981){2.12125}
\ECirc(44.2364,22.0578){0.775133}
\ECirc(-33.517,-33.6459){0.900842}
\ECirc(-8.62624,32.5595){1.00199}
\ECirc(-60.2216,18.846){2.12132}
\ECirc(-23.1603,2.09346){2.14578}
\ECirc(-21.8169,58.4696){1.45253}
\ECirc(-20.5668,51.3896){2.12111}
\ECirc(13.5349,-0.978575){1.16385}
\ECirc(38.4532,-1.62618){2.09965}
\ECirc(-25.9817,3.97283){0.87505}
\ECirc(-26.6018,8.00784){1.64026}
\ECirc(-48.7761,-22.1573){2.12045}
\ECirc(28.1709,-12.545){0.715713}
\ECirc(18.3131,-20.3386){0.858986}
\ECirc(16.0646,-21.2771){0.89511}
\ECirc(15.434,-20.9892){1.67179}
\ECirc(18.1376,-21.0055){0.512325}
\ECirc(12.3885,-34.5088){2.12131}
\ECirc(-4.43786,45.9272){1.46892}
\ECirc(-38.2105,-36.9209){2.12131}
\ECirc(-31.8997,-35.256){2.02376}
\ECirc(-52.3053,42.9371){1.44811}
\ECirc(-0.603031,-46.7928){1.37096}
\ECirc(-0.871538,-44.4792){2.00364}
\ECirc(3.18076,-43.6273){1.22336}
\ECirc(-28.0932,33.2175){2.11435}
\ECirc(-34.6176,35.3207){2.11963}
\ECirc(45.2308,28.4656){2.11633}
\ECirc(47.8245,22.974){1.21264}
\ECirc(42.0645,26.6895){1.22395}
\ECirc(47.3805,25.4653){2.12115}
\ECirc(17.7568,-8.19139){2.12129}
\ECirc(8.94815,-21.2764){2.12092}
\ECirc(18.8487,-52.4783){2.12132}
\ECirc(-13.1281,-48.1333){1.09058}
\ECirc(-2.51458,-8.62929){1.48583}
\ECirc(-37.9391,-2.22132){2.12132}
\ECirc(10.2403,-14.4324){2.29917}
\ECirc(6.99065,-10.6112){1.24502}
\ECirc(8.99848,-14.7228){0.564709}
\ECirc(9.98224,-19.5438){0.85373}
\ECirc(69.6529,15.9439){2.12121}
\ECirc(46.9502,-46.5553){2.10668}
\ECirc(-19.8064,-23.8336){2.11509}
\ECirc(8.37789,19.8709){2.08615}
\ECirc(-32.9374,30.5483){2.12132}
\ECirc(-37.2455,42.25){1.97448}
\ECirc(65.4827,-18.4693){1.59804}
\ECirc(4.39859,-14.6142){2.11535}
\ECirc(3.46942,-9.99601){1.66696}
\ECirc(2.96037,-10.4543){1.70556}
\ECirc(-0.117354,-8.16874){2.00753}
\ECirc(-2.68714,-4.43136){2.08413}
\ECirc(8.62463,-11.7632){1.04113}
\ECirc(5.7979,-13.1667){2.10952}
\ECirc(-6.46067,-24.8451){1.24259}
\ECirc(-4.84493,-27.9333){2.1205}
\ECirc(-3.7403,-29.4018){1.29309}
\ECirc(-2.2647,-23.2839){1.29874}
\ECirc(-3.16341,-24.7261){0.634175}
\ECirc(-4.29394,-25.9104){0.884297}
\ECirc(-2.95659,-23.4626){2.10136}
\ECirc(28.5655,59.0544){1.18182}
\ECirc(-18.4085,20.5598){2.11163}
\ECirc(-57.9608,15.0257){2.1029}
\ECirc(-59.287,22.3159){1.05944}
\ECirc(-51.2195,14.8041){0.50626}
\ECirc(-50.758,14.2721){0.687747}
\ECirc(-57.2912,21.0523){1.06012}
\ECirc(-9.33309,-35.4621){1.2879}
\ECirc(-3.73813,-52.8518){2.11483}
\ECirc(39.1283,-42.478){1.93436}
\ECirc(29.5775,66.5645){0.829607}
\ECirc(9.33435,8.02527){1.621}
\ECirc(19.5177,33.301){0.385503}
\ECirc(20.9319,28.2789){1.76369}
\ECirc(26.4566,16.5922){1.66166}
\ECirc(-18.0936,22.9833){1.88579}
\ECirc(-20.4289,24.447){2.02314}
\ECirc(-20.1883,24.1794){2.00262}
\ECirc(-17.5047,21.5025){1.25969}
\ECirc(-17.051,20.3225){1.54324}
\ECirc(27.8831,42.0069){0.95204}
\ECirc(-49.269,24.6686){1.5762}
\ECirc(27.1774,-21.3885){2.12112}
\ECirc(30.1801,-27.305){2.08945}
\ECirc(19.9999,4.5902){1.30599}
\ECirc(13.6283,3.10191){1.55008}
\ECirc(13.0532,10.1729){1.0744}
\ECirc(41.5554,-24.4911){1.86489}
\ECirc(44.6384,-22.8651){1.24907}
\ECirc(42.9155,-26.1825){1.91911}
\ECirc(42.913,-22.6606){2.12128}
\ECirc(42.672,-21.1986){2.12032}
\ECirc(65.3275,17.9042){2.11024}
\ECirc(-13.5614,-16.5694){1.12137}
\ECirc(-5.10504,-9.87818){1.46837}
\ECirc(-7.89381,-13.989){1.48375}
\ECirc(-17.6611,-11.4995){1.13219}
\ECirc(-61.5408,-18.9675){2.12132}
\ECirc(11.7443,-31.6889){1.56392}
\ECirc(12.0978,-30.5678){1.85213}
\ECirc(11.8351,-29.4896){2.09924}
\ECirc(4.89949,-28.9621){0.725966}
\ECirc(59.0096,28.5765){2.06872}
\ECirc(29.1551,10.0263){2.01034}
\ECirc(31.9518,15.1787){0.742406}
\ECirc(31.0036,16.0709){0.978537}
\ECirc(-65.2427,16.2659){2.12132}
\ECirc(-12.3063,64.3706){1.08264}
\ECirc(-32.7054,-33.2276){0.875331}
\ECirc(20.3179,31.4045){2.01298}
\ECirc(-23.2617,73.6246){1.67421}
\ECirc(-51.1298,-0.29012){0.965042}
\ECirc(-32.0023,-14.1288){2.12127}
\ECirc(-25.2259,-6.70837){2.12132}
\ECirc(-28.6272,-15.034){0.638308}


==> figs/PbPb-5.tex <==
\ECirc(-8.11415,-11.35){1.56128}
\ECirc(27.6499,28.9182){0.612132}
\ECirc(23.3375,-40.2258){3.40328}
\ECirc(15.8944,-36.8848){1.66851}
\ECirc(46.8121,-14.341){3.11856}
\ECirc(25.1524,-25.2591){2.19194}
\ECirc(-22.8488,-10.2707){2.38534}
\ECirc(25.6506,37.796){2.12585}
\ECirc(-3.45086,47.446){3.00724}
\ECirc(5.31255,-51.0515){3.52994}
\ECirc(4.36977,-50.923){3.13241}
\ECirc(21.3031,-22.6036){2.40326}
\ECirc(-21.1747,-24.6194){3.1687}
\ECirc(-28.1528,-47.1257){2.24353}
\ECirc(-21.8018,-43.053){2.881}
\ECirc(-58.2854,14.718){3.10793}
\ECirc(0.441121,-66.2903){3.2558}
\ECirc(36.0735,48.0488){3.17349}
\ECirc(-32.5651,3.4475){3.08069}
\ECirc(-24.9922,-9.62532){2.95056}
\ECirc(-25.799,19.8667){1.82876}
\ECirc(9.45776,-24.0266){0.594189}
\ECirc(8.96848,-2.08323){2.5827}
\ECirc(-14.4302,-28.4524){2.4748}
\ECirc(-9.61896,47.4043){3.46825}
\ECirc(6.79016,32.3548){1.73481}
\ECirc(6.70437,38.2443){3.52767}
\ECirc(16.1315,-48.9039){1.39903}
\ECirc(-34.576,-14.0895){3.32559}
\ECirc(27.0433,41.7217){2.88796}
\ECirc(25.089,34.8917){3.40449}
\ECirc(-38.4435,13.2134){3.02345}
\ECirc(31.2555,26.8523){1.801}
\ECirc(-24.2033,6.86197){3.26758}
\ECirc(25.2189,38.9529){1.8358}
\ECirc(-37.0738,-40.708){3.50276}
\ECirc(40.6942,-3.88211){0.499891}
\ECirc(-24.264,45.5814){3.44856}
\ECirc(4.04766,-53.279){3.09445}
\ECirc(-35.0744,-2.31294){2.07154}
\ECirc(26.7842,-15.6719){2.97414}
\ECirc(23.1994,-36.1912){2.30954}
\ECirc(8.8668,-48.6082){1.75319}
\ECirc(5.77844,-46.1425){2.37983}
\ECirc(-38.1368,-3.89963){0.883017}
\ECirc(-35.2183,-32.9414){1.66768}
\ECirc(15.8298,-45.2408){0.969661}
\ECirc(20.7372,29.3309){2.67126}
\ECirc(5.6628,57.9902){2.86075}
\ECirc(-6.96051,42.7444){1.20022}
\ECirc(-8.2471,42.2326){1.85576}
\ECirc(-0.455365,41.4044){2.71795}
\ECirc(-21.8053,-11.6593){3.18632}
\ECirc(11.2114,-46.2104){2.95214}
\ECirc(9.20256,-49.3265){1.7126}
\ECirc(4.01713,-14.0766){3.49844}
\ECirc(26.4197,10.3414){2.90479}
\ECirc(-40.6513,17.2126){2.23515}
\ECirc(-4.30583,-22.233){3.08995}
\ECirc(21.9092,-11.2884){3.27514}
\ECirc(-40.0794,32.7783){3.29531}
\ECirc(39.6152,-5.74554){0.878858}
\ECirc(48.9908,-26.0872){2.93817}
\ECirc(-0.654295,0.0606627){3.33716}
\ECirc(4.4415,-54.6138){1.75376}
\ECirc(4.15184,38.3816){2.93517}
\ECirc(4.51949,36.809){2.68133}
\ECirc(-4.67007,-6.50782){3.38572}
\ECirc(-23.5076,-15.983){0.683997}
\ECirc(6.60322,45.0276){2.67563}
\ECirc(-9.41965,-36.8268){3.41938}
\ECirc(-50.294,10.2528){2.58243}
\ECirc(-0.377981,-22.4309){3.52781}
\ECirc(19.5361,30.9039){3.35521}
\ECirc(-39.8069,41.9862){2.1038}
\ECirc(-39.0915,35.8251){2.57066}
\ECirc(21.8503,-40.8711){2.43282}
\ECirc(39.292,34.5106){3.28186}
\ECirc(6.78193,-5.91374){1.70319}
\ECirc(-32.4803,-5.36814){3.5206}
\ECirc(-15.0333,7.96932){2.75574}
\ECirc(28.4659,35.6833){3.52053}
\ECirc(9.48867,-11.229){1.69}
\ECirc(14.8504,-9.12838){2.23411}
\ECirc(-14.9542,-38.637){1.27976}
\ECirc(-13.1197,-1.00752){0.979582}
\ECirc(10.47,5.98931){3.00576}
\ECirc(-36.0796,11.7539){2.95335}
\ECirc(-34.6516,13.3847){1.00631}
\ECirc(-32.9043,4.81485){2.26662}
\ECirc(-16.0209,-42.3131){3.05018}
\ECirc(-12.6779,-28.9775){2.17536}
\ECirc(18.7714,-36.657){2.98817}
\ECirc(42.7937,7.60133){3.51051}
\ECirc(18.3065,-1.9556){3.41986}
\ECirc(-21.0837,-10.9785){3.37405}
\ECirc(17.0212,4.64755){1.20029}
\ECirc(-42.8363,-4.0775){3.46162}
\ECirc(29.937,18.9828){3.45053}
\ECirc(-51.9322,-27.2236){3.4579}
\ECirc(-39.2946,-8.362){3.50367}
\ECirc(-25.2331,-8.64756){1.34836}
\ECirc(7.69611,-49.5289){2.68496}
\ECirc(-19.2884,-21.6184){2.14656}
\ECirc(-1.49571,50.2186){3.26875}
\ECirc(-11.7805,-56.8381){3.55393}
\ECirc(27.4675,-9.47639){3.46013}
\ECirc(55.9475,-3.68473){3.50741}
\ECirc(59.06,-5.2256){1.97887}
\ECirc(59.5072,-4.55739){2.20466}
\ECirc(-5.29539,9.69299){1.49665}
\ECirc(22.7203,-34.3502){2.44094}
\ECirc(-45.219,7.11855){1.30736}
\ECirc(-2.65934,50.9114){3.25901}
\ECirc(7.86985,-30.5746){3.49021}
\ECirc(-60.5417,8.27707){3.26519}
\ECirc(-10.4499,49.7562){2.33415}
\ECirc(-12.144,50.7084){2.65454}
\ECirc(-14.9053,-24.2274){3.52237}
\ECirc(20.8715,-23.2377){3.51807}
\ECirc(-21.7149,-8.82233){2.36812}
\ECirc(44.6954,-32.4243){3.53468}
\ECirc(-8.94297,-7.53322){3.17364}
\ECirc(9.29303,34.8038){3.35462}
\ECirc(8.52751,39.3316){2.1255}
\ECirc(64.4969,-18.5489){3.13952}
\ECirc(-7.40539,14.5756){3.49113}
\ECirc(-2.45833,17.9081){3.27331}
\ECirc(-26.5535,42.0003){3.43124}
\ECirc(-21.1652,38.7849){1.83852}
\ECirc(-5.59326,11.6519){2.62834}
\ECirc(-5.72562,10.362){1.13885}
\ECirc(0.0355473,6.98412){1.43577}
\ECirc(-36.8974,-11.5935){0.938041}
\ECirc(-56.4324,40.9566){3.37889}
\ECirc(25.4979,31.2226){2.86864}
\ECirc(6.9521,-2.2378){1.24789}
\ECirc(1.68402,-6.49107){2.71059}
\ECirc(29.7856,23.4524){3.53344}
\ECirc(-16.7367,59.5755){1.4011}
\ECirc(3.28244,53.1949){3.42528}
\ECirc(-11.5618,-21.0142){3.23588}
\ECirc(-36.1318,-8.75232){3.00019}
\ECirc(-35.1734,-9.32848){3.30493}
\ECirc(29.5315,-24.8679){3.43757}
\ECirc(-1.0672,-3.21214){3.51564}
\ECirc(-8.92741,-8.74171){3.40804}
\ECirc(27.1084,5.51068){3.53176}
\ECirc(15.6611,-7.88877){3.06965}
\ECirc(3.6339,-1.37311){2.43656}
\ECirc(6.92697,6.32871){0.887627}
\ECirc(2.09281,5.10503){2.64905}
\ECirc(3.58044,-8.85469){3.4819}
\ECirc(24.7468,48.2586){2.56167}
\ECirc(41.7413,3.46326){3.51036}
\ECirc(25.8345,77.607){1.58642}
\ECirc(5.78736,35.5229){3.46046}
\ECirc(8.15241,-6.45192){2.18553}
\ECirc(-26.5373,-5.58426){3.07795}
\ECirc(-27.357,-4.19866){2.91822}
\ECirc(-23.4541,-0.848288){1.36592}
\ECirc(-29.604,-5.06635){3.43516}
\ECirc(-7.79844,42.1838){3.21527}
\ECirc(-11.034,41.7426){3.52846}
\ECirc(-12.9749,3.16679){3.4629}
\ECirc(12.829,-51.1242){3.53053}
\ECirc(5.18842,-0.854692){1.97328}
\ECirc(5.25779,-3.65446){3.4259}
\ECirc(49.4178,28.5577){3.47507}
\ECirc(-26.8027,26.4794){3.52844}
\ECirc(13.5698,-45.8261){1.07401}
\ECirc(-36.47,-41.7666){3.19327}
\ECirc(18.1301,-7.32553){3.51645}
\ECirc(21.2755,24.8525){0.946483}
\ECirc(-13.1557,-17.509){3.52174}
\ECirc(-42.5418,-11.224){3.41364}
\ECirc(23.8881,4.94554){3.43818}
\ECirc(40.3115,-2.03575){2.87052}
\ECirc(38.1299,-25.3276){2.09133}
\ECirc(49.1816,-0.368689){3.52714}
\ECirc(13.072,56.959){1.41472}
\ECirc(63.6309,16.113){3.33028}
\ECirc(58.1692,-5.3683){1.7611}
\ECirc(54.9547,-5.22102){2.82205}
\ECirc(-26.6725,-18.1568){3.0586}
\ECirc(3.23184,-54.9943){3.39759}
\ECirc(-3.8451,-5.88063){2.87756}
\ECirc(-1.13982,-1.49085){3.24765}
\ECirc(-6.47056,34.2861){3.5291}
\ECirc(6.94205,-50.4214){3.38117}
\ECirc(62.0316,-15.4919){1.68395}
\ECirc(10.7673,27.9942){1.98039}
\ECirc(52.7742,12.3318){1.28506}
\ECirc(59.6221,20.2761){1.8186}
\ECirc(51.8291,17.7564){3.52951}
\ECirc(26.8735,-12.1279){3.42734}
\ECirc(10.82,41.4552){3.12081}
\ECirc(62.3757,-21.547){3.53382}
\ECirc(-22.9484,-14.4463){2.37559}
\ECirc(40.4394,6.97666){3.13257}
\ECirc(1.02965,49.1717){1.50827}
\ECirc(0.715758,-43.3664){3.45186}
\ECirc(8.11896,2.80279){3.52676}
\ECirc(-12.6994,-6.45058){3.39988}
\ECirc(-14.5163,-32.3924){0.83034}
\ECirc(-11.4599,-33.4765){0.791869}
\ECirc(-12.042,-37.5906){1.38985}
\ECirc(-10.2838,-31.1888){1.48887}
\ECirc(-7.57967,-41.2592){1.53422}
\ECirc(-35.2897,46.5593){3.12838}
\ECirc(23.1006,0.984733){3.52637}
\ECirc(-32.8551,2.79774){1.90992}
\ECirc(-46.0607,-3.24303){0.993147}
\ECirc(45.8327,30.8268){3.26953}
\ECirc(40.0225,29.4569){2.61787}
\ECirc(39.927,31.1159){3.7191}
\ECirc(18.3358,7.91224){2.65516}
\ECirc(-36.0776,12.009){1.93178}
\ECirc(-33.9102,22.1601){1.34042}
\ECirc(-33.6388,20.329){1.11447}
\ECirc(-33.4849,18.344){0.829548}
\ECirc(-7.76528,-27.5131){1.98133}
\ECirc(49.684,33.4986){0.886864}
\ECirc(50.4138,34.6037){2.36959}
\ECirc(-50.474,-9.38344){1.63752}
\ECirc(-45.6233,-3.89362){1.55076}
\ECirc(-26.205,21.151){3.19234}
\ECirc(-42.4622,-28.6744){3.01945}
\ECirc(-49.7297,-25.0559){3.51611}
\ECirc(41.3873,-37.1364){2.26616}
\ECirc(-40.7488,31.5252){1.93505}
\ECirc(-22.007,-8.39746){2.07355}
\ECirc(-45.9172,-14.5822){3.47458}
\ECirc(17.1805,-59.3603){1.34224}
\ECirc(15.2767,-53.8613){3.45244}
\ECirc(1.79912,14.903){3.44542}
\ECirc(17.2091,-46.8318){2.55157}
\ECirc(15.2151,-44.2887){1.88479}
\ECirc(21.1267,60.0601){3.32484}
\ECirc(21.539,61.2357){3.41172}
\ECirc(4.85711,7.13555){2.90303}
\ECirc(4.3473,12.2379){3.03189}
\ECirc(5.7475,-15.4535){3.52741}
\ECirc(-18.8667,16.4157){1.76268}
\ECirc(-3.57902,-11.3379){0.513424}
\ECirc(-4.3353,-18.36){1.68824}
\ECirc(-4.88079,-14.1954){3.00744}
\ECirc(26.6136,-17.7078){2.07278}
\ECirc(4.36716,14.4055){1.73058}
\ECirc(3.2731,-0.698636){3.5012}
\ECirc(-24.5994,46.3229){0.845393}
\ECirc(-47.4371,-13.7466){3.42113}
\ECirc(-35.4227,-34.964){1.42171}
\ECirc(2.62193,59.2773){2.8523}
\ECirc(12.6181,-44.192){1.82744}
\ECirc(10.8943,-34.2864){2.44362}
\ECirc(7.97605,0.692384){3.53539}
\ECirc(63.2352,-19.372){3.46753}
\ECirc(-33.4787,-47.8004){2.57749}
\ECirc(-33.4144,-46.9895){2.66368}
\ECirc(48.3385,28.9743){3.25822}
\ECirc(45.2679,28.959){1.35144}
\ECirc(49.9897,-39.0562){3.24593}
\ECirc(50.873,-34.4731){2.67478}
\ECirc(0.43926,11.7411){2.90691}
\ECirc(-47.6567,-11.7677){3.53366}
\ECirc(16.0198,-32.1748){3.49181}
\ECirc(17.2474,-35.0924){2.64056}
\ECirc(18.2642,-31.3556){3.21333}
\ECirc(-12.3743,-21.8807){3.52287}
\ECirc(28.2192,32.0389){3.53428}
\ECirc(-16.3738,-0.638788){2.23529}
\ECirc(-40.9055,2.35717){3.06992}
\ECirc(58.6439,-3.15975){3.53141}
\ECirc(39.0104,-1.29431){3.19477}
\ECirc(39.0356,-0.895235){2.95581}
\ECirc(18.4446,-12.9913){3.51182}
\ECirc(-36.0543,-6.01565){3.53364}
\ECirc(13.172,-4.48355){3.5149}
\ECirc(-34.2624,19.5156){3.04254}
\ECirc(-31.0484,20.1499){1.21122}
\ECirc(34.9995,-46.9167){3.28903}
\ECirc(-10.0557,11.8748){1.95597}
\ECirc(-9.60827,10.4414){1.8531}
\ECirc(-7.37993,7.34763){0.399487}
\ECirc(-17.8904,-20.7604){2.99858}
\ECirc(-38.5527,15.2223){2.03252}
\ECirc(-34.2253,8.64624){2.44599}
\ECirc(26.6926,29.1125){1.79948}
\ECirc(4.77451,1.76447){3.55873}
\ECirc(-19.4874,-25.532){2.21051}
\ECirc(9.79798,3.95997){3.47582}
\ECirc(25.2837,31.4529){3.6405}
\ECirc(0.680361,54.8115){2.95082}
\ECirc(-35.4156,2.07609){0.922799}
\ECirc(-35.1665,3.15956){0.953039}
\ECirc(3.27175,51.3589){2.64576}
\ECirc(-21.3594,-16.3859){3.3711}
\ECirc(35.7894,-2.92199){2.66964}
\ECirc(34.7881,2.77942){0.81086}
\ECirc(-5.15486,46.4863){3.51993}
\ECirc(21.1139,19.9149){0.473047}
\ECirc(21.6576,16.3508){0.358617}
\ECirc(21.706,24.0245){3.52856}
\ECirc(30.6995,24.1537){1.54046}
\ECirc(56.2221,35.1903){0.81071}
\ECirc(-15.5199,-21.5581){2.11969}
\ECirc(-24.8323,-18.6862){1.99682}
\ECirc(-17.2767,2.90748){3.54405}
\ECirc(26.1279,-5.88494){3.4117}
\ECirc(21.9058,-21.3592){3.49595}
\ECirc(-53.9518,2.74437){1.51168}
\ECirc(-47.9802,5.75727){1.59441}
\ECirc(5.35591,-0.860088){1.8357}
\ECirc(11.3889,1.18969){2.80359}
\ECirc(21.1743,-38.3214){3.53281}
\ECirc(8.49483,31.3688){1.62152}
\ECirc(6.85726,33.4088){1.72903}
\ECirc(-16.0739,12.6879){2.64076}
\ECirc(-29.6717,-22.7586){2.99945}
\ECirc(47.4817,-6.93953){2.38431}
\ECirc(44.0235,-7.27233){2.34521}
\ECirc(43.8432,-7.11677){2.80447}
\ECirc(47.0688,-9.967){3.39944}
\ECirc(-40.6861,-29.4071){3.37058}
\ECirc(-42.262,-29.9465){2.86359}
\ECirc(-9.26605,-8.13263){1.38032}
\ECirc(19.3428,32.9669){2.89736}
\ECirc(19.6266,-37.0121){3.19961}
\ECirc(25.4248,-38.2437){3.37687}
\ECirc(29.4631,-36.0982){3.28184}
\ECirc(31.6252,31.4766){1.94632}
\ECirc(-8.70588,-0.144598){3.45895}
\ECirc(13.8486,-17.4577){3.22829}
\ECirc(-25.8187,49.9229){2.06398}
\ECirc(-30.1979,46.9099){2.76112}
\ECirc(-17.1956,-9.39278){1.18461}
\ECirc(7.8979,1.28598){3.41445}
\ECirc(27.7541,21.0773){3.39811}
\ECirc(-1.86344,-3.59727){2.43548}
\ECirc(49.3968,-12.6205){3.68779}
\ECirc(3.34403,-24.6935){1.76123}
\ECirc(4.44938,-30.3352){3.18301}
\ECirc(-8.08741,7.03436){2.92358}
\ECirc(16.9823,-51.9223){1.79139}
\ECirc(11.0619,-51.1132){2.73687}
\ECirc(10.187,-49.4715){2.73827}
\ECirc(17.7807,-19.4868){3.23793}
\ECirc(23.5036,-27.9679){0.877867}
\ECirc(-44.4572,1.84057){3.53419}
\ECirc(12.6455,-25.6223){1.80109}
\ECirc(3.19197,-28.1612){3.51232}
\ECirc(4.42892,-23.0371){1.52906}
\ECirc(11.4558,-26.5695){1.26292}
\ECirc(12.0616,-2.30902){3.52595}
\ECirc(35.2735,-47.3473){3.19958}
\ECirc(31.7453,-43.2656){3.09724}
\ECirc(-8.10907,-37.7139){3.52883}
\ECirc(1.92581,14.2697){1.33646}
\ECirc(12.5303,-27.1507){3.52577}
\ECirc(12.7109,-25.6365){3.03543}
\ECirc(17.8109,-23.2584){2.99426}
\ECirc(16.13,-18.3681){1.55585}
\ECirc(-5.90066,-58.0267){3.53478}
\ECirc(40.8958,2.81708){3.51122}
\ECirc(43.0585,1.97951){2.58175}
\ECirc(45.6183,1.90756){1.72357}
\ECirc(-32.1341,-26.3716){3.15699}
\ECirc(4.31798,-13.6058){3.53075}
\ECirc(15.9857,-56.6234){3.27031}
\ECirc(-2.97865,24.8402){3.20123}
\ECirc(-38.3849,1.44694){1.56474}
\ECirc(19.6726,-9.45053){2.48077}
\ECirc(14.8534,-7.27036){4.73904}
\ECirc(19.5282,-16.5577){1.10854}
\ECirc(33.193,29.4797){3.50817}
\ECirc(33.6304,30.5){3.5138}
\ECirc(46.7214,-10.7233){3.53257}
\ECirc(-12.1391,45.0709){3.50048}
\ECirc(-10.3392,-27.7356){1.19624}
\ECirc(0.235658,-5.08805){3.43949}
\ECirc(3.70985,-4.34172){3.51834}
\ECirc(58.3345,-5.34194){0.750616}
\ECirc(-14.2069,-55.4569){3.48582}
\ECirc(-43.4854,38.8296){3.50759}
\ECirc(-49.8956,37.7716){2.92209}
\ECirc(-49.9197,38.9828){2.76633}
\ECirc(-47.719,32.4512){3.44533}
\ECirc(-7.26619,-2.31352){1.87369}
\ECirc(28.5306,29.9049){3.43012}
\ECirc(33.7016,-40.0249){3.15749}
\ECirc(42.4403,-45.2234){3.03779}
\ECirc(44.5101,-43.1025){3.11295}
\ECirc(1.53523,25.8557){3.52854}
\ECirc(-6.83655,-36.1872){3.53288}
\ECirc(15.4831,-3.28327){3.49808}
\ECirc(-15.1152,-36.0045){3.52535}
\ECirc(28.9251,20.3363){3.53301}
\ECirc(52.4363,0.0399088){0.791886}
\ECirc(55.3129,2.28415){1.75674}
\ECirc(57.469,5.21057){0.6683}
\ECirc(11.0282,8.61397){0.917678}
\ECirc(-20.4321,-18.5705){3.53413}
\ECirc(-3.90058,7.25768){3.42402}
\ECirc(-1.80407,0.119643){3.53235}
\ECirc(59.3145,-13.0828){3.22864}
\ECirc(-20.0925,7.43256){0.212479}
\ECirc(-19.2134,5.94563){1.56935}
\ECirc(-39.0214,-32.3173){3.28136}
\ECirc(-29.3068,-5.74557){3.5867}
\ECirc(18.0407,-6.40594){2.70533}
\ECirc(55.0172,43.9761){3.51225}
\ECirc(51.3881,43.1028){3.05014}
\ECirc(7.63799,-15.1458){3.48253}
\ECirc(-45.4799,9.36485){1.93064}
\ECirc(-35.4889,40.2753){1.49769}
\ECirc(-40.0479,1.26033){3.4492}
\ECirc(-40.4601,1.05781){2.92034}
\ECirc(50.2356,44.0644){3.51613}
\ECirc(-32.383,26.2853){2.03522}
\ECirc(3.77485,-2.36078){3.54734}
\ECirc(12.1145,2.57527){3.53224}
\ECirc(13.2618,5.9328){3.46331}
\ECirc(18.7852,15.6526){1.63384}
\ECirc(-7.14012,-38.0349){3.47865}
\ECirc(-11.7066,-10.1217){2.00619}
\ECirc(-6.03345,-15.4984){3.36152}
\ECirc(-43.2627,-16.28){3.51711}
\ECirc(-26.3455,-29.8961){2.81631}
\ECirc(-2.89256,-18.7037){3.47956}
\ECirc(-31.9509,-20.3353){3.39724}
\ECirc(53.245,14.0962){3.47682}
\ECirc(-13.5038,-56.1499){3.45755}
\ECirc(-19.6094,54.2269){1.53883}
\ECirc(2.00504,-19.8976){1.49581}
\ECirc(-3.96453,-5.9293){3.53255}
\ECirc(-13.42,-3.29125){3.40706}
\ECirc(-7.63892,-4.47506){3.3639}
\ECirc(44.6385,29.9905){3.45978}
\ECirc(-14.4571,-54.0003){3.50939}
\ECirc(24.9702,35.4005){3.53457}
\ECirc(45.2295,-17.5483){2.43555}
\ECirc(45.43,-13.5439){0.709656}
\ECirc(48.3046,-15.5322){1.18416}
\ECirc(44.2495,-20.1192){1.25335}
\ECirc(46.1344,-7.80691){3.01425}
\ECirc(51.5249,-7.8199){1.89168}
\ECirc(53.2886,-15.034){3.24603}
\ECirc(51.9738,-15.3326){2.76716}
\ECirc(10.6133,-2.86674){3.51791}
\ECirc(12.2676,7.7606){1.2431}
\ECirc(-53.4325,33.454){3.53492}
\ECirc(-13.159,2.98011){3.25534}
\ECirc(-43.3579,7.19605){3.5345}
\ECirc(18.0638,28.4484){1.73845}
\ECirc(24.6105,34.2016){3.13473}
\ECirc(16.2045,36.2184){2.69637}
\ECirc(22.7679,39.4208){2.55836}
\ECirc(-56.5047,-19.9133){1.07058}
\ECirc(-53.8839,-24.0664){2.06911}
\ECirc(-44.1685,-16.4982){0.520922}
\ECirc(-11.7091,-19.8465){3.47855}
\ECirc(21.7185,-37.455){3.33689}
\ECirc(42.1035,-3.25378){3.40686}
\ECirc(6.32548,-47.1453){3.53533}
\ECirc(6.75634,-57.4778){3.03339}
\ECirc(-57.9237,20.4393){3.64216}
\ECirc(-56.0878,19.3623){1.10482}
\ECirc(-11.0967,6.72897){3.51809}
\ECirc(-2.74244,16.6101){3.05773}
\ECirc(2.26065,15.0996){3.48307}
\ECirc(-10.8799,48.1942){3.11419}
\ECirc(-7.77409,47.9587){1.53731}
\ECirc(-26.5249,35.4194){3.44178}
\ECirc(-28.4286,39.122){1.60095}
\ECirc(24.8483,-36.8505){1.77549}
\ECirc(-18.0825,-43.61){2.6929}
\ECirc(-10.078,-43.69){2.5838}
\ECirc(36.3618,39.8715){3.52275}
\ECirc(12.1714,-43.5445){3.51334}
\ECirc(4.21232,-17.4525){3.53269}
\ECirc(38.4103,23.7178){2.61914}
\ECirc(-11.9758,-21.6852){3.53477}
\ECirc(-26.47,30.533){2.61296}
\ECirc(-46.2994,-8.24037){3.53498}
\ECirc(-21.3498,21.4109){0.498826}
\ECirc(-21.1298,26.2545){0.559293}
\ECirc(36.771,-2.66426){3.48795}
\ECirc(38.9674,-5.1115){3.39125}
\ECirc(-45.6805,-25.1699){2.99758}
\ECirc(-35.8743,43.9522){3.5052}
\ECirc(53.3176,35.0689){3.51585}
\ECirc(-56.7261,36.5104){3.52666}
\ECirc(61.2709,18.1287){3.50322}
\ECirc(51.6892,40.7955){3.53315}
\ECirc(17.5667,23.2257){3.53688}
\ECirc(14.6026,-57.1603){3.53534}
\ECirc(-52.9247,1.99464){2.84481}
\ECirc(-2.1814,-2.83895){2.17311}
\ECirc(1.49183,-1.55784){3.07951}
\ECirc(3.1434,3.06169){3.09357}
\ECirc(-6.976,23.5567){3.26015}
\ECirc(-5.51998,32.4228){2.68318}
\ECirc(22.0506,-11.88){3.53196}
\ECirc(-22.4565,19.103){3.52928}
\ECirc(-21.3099,6.34713){3.25364}
\ECirc(15.7727,27.9602){2.20382}
\ECirc(15.4928,26.9124){3.49192}
\ECirc(-18.3865,-16.1422){3.53521}
\ECirc(-25.5649,5.73017){3.3989}
\ECirc(-19.4781,18.8433){3.58505}
\ECirc(50.1124,-16.2875){3.24757}
\ECirc(30.9437,-28.746){3.36258}
\ECirc(-12.1752,-39.9797){3.53503}
\ECirc(-40.2686,16.9197){3.29475}
\ECirc(29.5325,8.39485){2.82446}
\ECirc(-19.0713,-50.8899){3.38638}
\ECirc(-19.1381,10.3045){3.48005}
\ECirc(-27.2342,0.862503){2.44947}
\ECirc(-23.3099,6.03724){3.52841}
\ECirc(-30.1635,5.88121){2.23961}
\ECirc(3.74362,-21.9533){2.5326}
\ECirc(-29.4103,-5.45767){1.15141}
\ECirc(53.9208,-10.2414){3.52354}
\ECirc(-10.7413,-4.56003){3.48482}
\ECirc(-48.851,6.52846){5}
\ECirc(-3.09717,44.4912){3.5299}
\ECirc(-25.2026,14.5658){0.798146}
\ECirc(-21.3972,21.8451){3.53463}
\ECirc(-10.8056,-38.4079){3.5242}
\ECirc(1.70455,-2.29815){3.53532}
\ECirc(14.8769,5.12241){3.13944}
\ECirc(12.8456,8.55983){0.805505}
\ECirc(13.0026,8.79577){0.703346}
\ECirc(12.2448,3.39438){3.29227}
\ECirc(-21.648,-5.94028){3.53192}
\ECirc(-39.9922,44.7708){1.27694}
\ECirc(-41.5632,46.7604){1.84468}
\ECirc(-32.4851,45.3155){1.52361}
\ECirc(22.8285,14.4702){3.51056}
\ECirc(29.5768,12.0905){1.58996}
\ECirc(36.668,-38.2871){3.53543}
\ECirc(-51.3018,38.6026){2.10424}
\ECirc(18.2925,-35.0297){3.527}
\ECirc(39.881,9.32202){2.63245}
\ECirc(42.4667,11.174){2.94662}
\ECirc(44.3788,8.50484){3.44977}
\ECirc(46.4851,-0.861519){3.33258}
\ECirc(-8.82111,-5.46175){3.54164}
\ECirc(-35.2865,-14.5235){3.53551}
\ECirc(36.347,-30.033){3.53537}
\ECirc(-65.217,8.39266){2.45102}
\ECirc(-53.958,31.0767){2.60056}
\ECirc(-50.6153,33.4746){3.1851}
\ECirc(-48.1721,37.1138){3.04412}
\ECirc(-54.2831,21.3463){2.46737}
\ECirc(-56.3482,18.7722){3.23828}
\ECirc(17.954,-39.2315){3.53448}
\ECirc(-21.8432,44.2296){1.52784}
\ECirc(-30.9603,41.8855){1.12327}
\ECirc(-32.514,43.5629){0.848534}
\ECirc(47.8452,-34.6308){1.93803}
\ECirc(44.4278,-36.082){0.815455}
\ECirc(44.4589,-34.4678){1.04595}
\ECirc(50.3565,-36.7543){2.92312}
\ECirc(2.82259,-12.5571){2.60355}
\ECirc(3.97174,-11.3973){3.33709}
\ECirc(4.70037,-9.17061){3.45432}
\ECirc(9.506,-11.6841){2.77928}
\ECirc(7.52998,-13.2983){3.12612}
\ECirc(7.53716,-6.14366){2.91779}
\ECirc(14.8455,-12.903){1.76376}
\ECirc(18.5082,-14.0686){1.9712}
\ECirc(51.5367,-28.5864){3.51854}
\ECirc(46.679,-30.9189){1.59846}
\ECirc(46.3507,-31.2352){1.25694}
\ECirc(50.6544,-34.3295){1.06027}
\ECirc(6.78643,7.68854){3.41828}
\ECirc(9.38249,0.511559){3.47917}
\ECirc(-31.049,-17.8832){3.53539}
\ECirc(-17.7189,-48.6733){1.76233}
\ECirc(-12.28,-43.8988){1.93139}
\ECirc(-11.2546,-43.6257){1.27614}
\ECirc(-17.069,-43.3012){2.00547}
\ECirc(23.8146,-24.8091){3.37795}
\ECirc(-28.7749,20.9114){3.5713}
\ECirc(-8.59393,-21.3505){3.05662}
\ECirc(-28.4874,30.3706){3.50976}
\ECirc(16.5013,-32.9442){3.52134}
\ECirc(5.05597,-30.1863){2.15987}
\ECirc(7.26104,-30.3193){3.51705}
\ECirc(-20.5309,12.5693){3.51772}
\ECirc(-23.2147,11.3913){2.30023}
\ECirc(-57.3105,-28.3464){3.49979}
\ECirc(12.1051,-35.7443){3.53424}
\ECirc(30.6591,37.0285){3.3052}
\ECirc(10.643,-49.1311){3.52852}
\ECirc(15.2105,-49.6516){3.53377}
\ECirc(-25.399,30.6){3.37094}
\ECirc(-30.8169,35.3223){3.51271}
\ECirc(-29.6767,33.1462){2.45788}
\ECirc(-31.2722,30.5941){1.66623}
\ECirc(24.1183,68.2253){2.75686}
\ECirc(22.8031,69.9534){1.8476}
\ECirc(21.1606,70.2776){2.32326}
\ECirc(20.9995,-42.1167){3.5354}
\ECirc(-16.7184,-11.7055){3.53422}
\ECirc(27.4949,29.7386){3.32812}
\ECirc(55.899,37.5165){0.885459}
\ECirc(38.3221,27.786){3.52868}
\ECirc(46.8206,28.4891){2.14}
\ECirc(49.078,-25.2764){3.25342}
\ECirc(20.1785,30.5504){3.53478}
\ECirc(22.462,32.6023){1.1854}
\ECirc(-5.70053,8.52762){1.04435}
\ECirc(-6.3085,7.27216){1.02497}
\ECirc(-6.47548,10.3629){1.56183}
\ECirc(10.956,-26.9957){3.50022}
\ECirc(10.2727,-21.3756){2.58127}
\ECirc(6.91393,-24.9939){1.15931}
\ECirc(6.77803,-25.5596){0.787632}
\ECirc(-25.8517,-21.8738){3.5354}
\ECirc(8.94131,-62.1845){3.53422}
\ECirc(10.5154,1.48603){1.59559}
\ECirc(18.15,-27.6328){2.64842}
\ECirc(23.0492,-29.6864){1.3055}
\ECirc(55.5278,40.4506){1.17425}
\ECirc(53.3766,35.2158){3.51515}
\ECirc(30.2702,10.3427){3.2156}
\ECirc(-33.8874,13.6562){0.982527}
\ECirc(41.4341,11.0533){3.28171}
\ECirc(38.666,14.6066){1.53812}
\ECirc(39.9475,15.2576){1.6144}
\ECirc(-16.6809,-28.5404){3.37761}
\ECirc(-16.1543,-29.6734){3.50206}
\ECirc(-44.7289,-10.3936){3.53271}
\ECirc(7.60556,-33.5589){3.53538}
\ECirc(-6.10716,-12.6001){3.53321}
\ECirc(-9.42432,-5.77871){1.09567}
\ECirc(-6.94706,-1.28246){2.74335}
\ECirc(-6.31765,-5.19627){3.39139}
\ECirc(-14.9359,-2.17594){2.44394}
\ECirc(-10.8056,-36.5546){3.12524}
\ECirc(-10.5038,-38.0121){3.32034}
\ECirc(43.5869,-10.1448){3.534}
\ECirc(46.4465,-11.5287){3.11336}
\ECirc(-7.93532,-3.61572){1.33046}
\ECirc(-36.5356,4.32304){3.53703}
\ECirc(-35.4946,1.67223){1.34789}
\ECirc(-43.0379,-3.48305){3.06312}
\ECirc(-16.9529,23.3802){3.53168}
\ECirc(-15.8764,21.8357){2.32956}
\ECirc(-52.2849,30.5581){3.11604}
\ECirc(-53.9406,31.615){3.51896}
\ECirc(63.9094,-18.1371){2.28557}
\ECirc(-24.0659,-4.41061){3.46312}
\ECirc(-15.3828,-11.3276){2.06396}
\ECirc(-18.1505,-5.0179){1.86356}
\ECirc(-17.8862,-3.0099){1.07001}
\ECirc(26.7265,-41.5262){1.26223}
\ECirc(22.0435,-44.1071){1.2182}
\ECirc(20.5941,-44.557){0.909265}
\ECirc(-47.6244,38.1755){3.53382}
\ECirc(-13.4717,12.7337){1.53464}
\ECirc(-32.8153,9.20263){1.85082}
\ECirc(41.5995,-34.6038){3.51996}
\ECirc(54.8809,-30.4345){2.49675}
\ECirc(7.88587,-46.2528){3.49676}
\ECirc(-20.7462,-5.65187){3.18994}
\ECirc(-20.9527,-9.95156){1.85939}
\ECirc(-16.844,-13.4875){1.286}
\ECirc(-17.2541,-10.4023){1.00364}
\ECirc(-14.6497,-16.0422){3.53368}
\ECirc(61.5663,-10.4308){3.53307}
\ECirc(-34.9176,-1.04421){0.839791}
\ECirc(6.88234,-0.446387){3.54778}
\ECirc(-16.4654,-33.1409){3.53545}
\ECirc(6.53091,36.272){3.53518}
\ECirc(2.80824,37.6155){2.32932}
\ECirc(67.9707,-20.2987){3.53337}
\ECirc(-53.6353,8.47831){3.50614}
\ECirc(-19.4337,-18.9733){3.53275}
\ECirc(11.1862,-50.8484){3.49487}
\ECirc(8.31454,-48.6578){2.63657}
\ECirc(19.3713,-55.7895){3.53537}
\ECirc(-39.0961,42.0668){2.97088}
\ECirc(-35.456,40.7196){2.90336}
\ECirc(45.565,36.059){1.42999}
\ECirc(-34.4632,12.3594){2.8849}
\ECirc(-47.9086,35.6574){1.7643}
\ECirc(-6.24897,-39.3278){3.4351}
\ECirc(-7.74996,-33.8177){1.65115}
\ECirc(-8.22509,-38.5554){1.53307}
\ECirc(-1.04902,-1.04858){3.52522}
\ECirc(-59.9983,14.3481){3.53861}
\ECirc(51.6807,-35.0198){1.11733}
\ECirc(48.9623,-39.2564){0.942412}
\ECirc(43.6419,-32.535){0.988379}
\ECirc(-15.1498,1.34535){3.52112}
\ECirc(30.8618,-40.3035){3.53198}
\ECirc(28.9774,-44.0924){2.37969}
\ECirc(27.3671,-42.5434){2.63716}
\ECirc(-32.0018,14.5769){1.15684}
\ECirc(-57.0712,18.7256){3.53459}
\ECirc(46.712,36.4284){3.5346}
\ECirc(43.8505,30.7743){3.30561}
\ECirc(17.9752,42.9388){3.54015}
\ECirc(9.35551,-48.0071){3.53546}
\ECirc(-51.2259,7.27265){2.80021}
\ECirc(-47.905,27.0043){0.770266}
\ECirc(-53.3002,25.3354){1.20501}
\ECirc(-48.1881,22.1434){1.53684}
\ECirc(-47.7216,18.859){1.50758}
\ECirc(-8.80718,-23.4758){3.53545}
\ECirc(11.0435,-54.7969){1.46634}
\ECirc(-36.3396,-10.695){1.74363}
\ECirc(-39.1083,-8.30846){3.53455}
\ECirc(-54.1908,25.7527){3.53549}
\ECirc(-13.9789,-51.6618){3.53443}
\ECirc(6.56148,-37.9433){3.51308}
\ECirc(-22.7884,18.6911){3.53496}
\ECirc(-29.8122,-30.149){1.84194}
\ECirc(-26.5111,-34.3366){2.85492}
\ECirc(-32.7199,-18.1518){2.0687}
\ECirc(3.39622,-14.6183){1.82312}
\ECirc(4.34034,-33.3653){0.895515}
\ECirc(-11.531,28.267){3.45995}
\ECirc(-13.3945,29.8334){3.53097}
\ECirc(-49.7786,26.8961){3.08399}
\ECirc(6.27137,8.78638){3.52089}
\ECirc(8.95941,-49.1323){3.37872}
\ECirc(-31.3823,4.30065){3.53546}
\ECirc(19.2203,-20.5776){1.08715}
\ECirc(20.2543,-6.94452){1.90959}
\ECirc(24.7629,-8.55042){2.14168}
\ECirc(-6.60344,-17.129){3.5355}
\ECirc(0.835696,3.55524){3.56133}
\ECirc(9.56789,3.16907){3.53562}
\ECirc(17.9167,25.426){0.754735}
\ECirc(2.07351,29.6379){3.54104}
\ECirc(-12.4656,39.3124){3.52924}
\ECirc(-18.4811,40.7492){1.91999}
\ECirc(-8.83654,40.2502){2.81687}
\ECirc(42.0384,-39.8207){1.25045}
\ECirc(-10.7876,-7.13711){3.53548}
\ECirc(-55.8641,16.5721){3.53809}
\ECirc(-33.8367,-6.41572){3.53033}
\ECirc(5.30564,25.7728){3.5306}
\ECirc(47.3444,-52.7588){2.84512}
\ECirc(-7.69188,24.9936){3.53411}
\ECirc(47.7196,13.5085){3.53412}
\ECirc(12.7036,-32.5754){0.587591}
\ECirc(8.15157,-32.3737){1.20219}
\ECirc(-9.30827,-49.5102){1.99428}
\ECirc(-5.87644,-48.2535){2.73462}
\ECirc(-6.31203,-47.1988){1.97971}
\ECirc(-9.39921,-50.5507){2.88464}
\ECirc(-6.10169,-51.1815){3.03892}
\ECirc(-3.45486,-53.336){3.53537}
\ECirc(13.7044,-47.751){1.76637}
\ECirc(13.4728,-49.6376){2.58161}
\ECirc(12.2693,-52.0379){3.29405}
\ECirc(13.4428,-52.0609){1.70138}
\ECirc(13.5282,-19.2552){3.53543}
\ECirc(-22.1506,-24.8341){3.53531}
\ECirc(-5.05175,1.47605){3.52595}
\ECirc(50.081,29.4258){0.939029}
\ECirc(2.06943,52.9082){3.53442}
\ECirc(47.0349,-10.0748){3.53447}
\ECirc(21.2336,-0.390461){3.53639}
\ECirc(-43.5565,-9.47763){2.03771}
\ECirc(-43.9859,-12.4852){1.23628}
\ECirc(-45.1172,-14.4595){1.0882}
\ECirc(-25.6619,33.4825){2.51508}
\ECirc(-24.3461,30.3725){2.49657}
\ECirc(-20.2265,41.0394){3.25753}
\ECirc(61.5589,-17.5486){3.53553}
\ECirc(3.53102,-3.67829){3.52384}
\ECirc(-0.283172,18.1909){3.32192}
\ECirc(2.22799,17.6924){3.52705}
\ECirc(-39.5325,-6.79058){3.53181}
\ECirc(41.5271,2.69897){3.53306}
\ECirc(28.0139,28.6857){2.63884}
\ECirc(-2.20175,-25.5908){3.53549}
\ECirc(21.1351,-10.8261){3.53499}
\ECirc(-0.808603,21.7992){2.66502}
\ECirc(-37.2585,0.974015){2.99449}
\ECirc(-38.8459,11.844){1.64583}
\ECirc(9.76499,-6.11118){3.53546}
\ECirc(-6.23868,-9.61498){3.53538}
\ECirc(-18.907,5.56615){2.42307}
\ECirc(-15.4416,-11.8318){3.53552}
\ECirc(26.6898,-12.7215){3.53523}
\ECirc(-21.4131,-21.6768){3.24662}
\ECirc(-35.4286,-35.2936){3.53387}
\ECirc(-30.1208,36.3306){3.53539}
\ECirc(16.7866,-10.3491){1.14315}
\ECirc(17.7963,-9.13126){2.95723}
\ECirc(29.8881,-12.801){0.373883}
\ECirc(25.4598,-14.4394){1.80826}
\ECirc(25.2966,-9.86932){1.43956}
\ECirc(8.73877,-19.6859){1.33244}
\ECirc(10.0633,-24.8461){2.26923}
\ECirc(10.1701,-25.6566){1.32013}
\ECirc(9.17671,-26.0564){3.53367}
\ECirc(10.5245,36.0295){1.45849}
\ECirc(6.43817,34.0686){1.29621}
\ECirc(2.48704,37.3607){1.00742}
\ECirc(2.44046,37.8051){0.712887}
\ECirc(9.70727,-53.4855){3.53435}
\ECirc(10.7981,-21.2759){3.53551}
\ECirc(-27.8689,-11.8152){3.53517}
\ECirc(-0.487563,53.8818){3.53587}
\ECirc(-0.0805711,14.2935){2.12627}
\ECirc(-2.04651,17.0451){3.21853}
\ECirc(-48.2321,25.7338){2.73944}
\ECirc(-48.1799,21.8713){2.38457}
\ECirc(-43.3429,23.8439){2.14128}
\ECirc(-43.1761,28.3239){1.3344}
\ECirc(-44.0026,28.5993){1.00222}
\ECirc(-16.6572,-9.90375){3.53541}
\ECirc(-19.8497,17.4297){1.61315}
\ECirc(-32.5567,15.5119){1.39432}
\ECirc(-28.7337,17.9082){2.14958}
\ECirc(18.9222,-36.2856){0.556198}
\ECirc(5.2467,31.5058){3.51878}
\ECirc(4.77197,35.4332){0.816638}
\ECirc(5.43154,34.4043){0.328953}
\ECirc(5.60078,33.985){0.328953}
\ECirc(23.3713,22.4735){2.74532}
\ECirc(19.5878,24.1476){3.53327}
\ECirc(20.634,34.7798){0.477121}
\ECirc(-40.5417,-30.6835){3.53512}
\ECirc(-39.711,3.53406){1.02083}
\ECirc(-0.82755,2.19354){3.5301}
\ECirc(27.7169,31.8147){1.19191}
\ECirc(25.714,28.6728){1.25655}
\ECirc(-32.893,-15.0343){3.53553}
\ECirc(-5.09152,-16.0233){3.56753}
\ECirc(34.8572,-26.3141){3.33181}
\ECirc(-39.8809,-28.3699){2.85744}
\ECirc(-44.2588,-20.6358){3.13002}
\ECirc(0.0668285,-13.0039){2.96348}
\ECirc(22.7041,44.3838){3.53326}
\ECirc(-34.0677,37.9938){3.52963}
\ECirc(17.0147,7.81609){2.98721}
\ECirc(55.5561,8.19872){2.54423}
\ECirc(60.1294,10.3475){2.16317}
\ECirc(55.6562,11.8641){1.81212}
\ECirc(-35.4557,30.9099){3.0965}
\ECirc(-27.7814,29.941){3.53442}
\ECirc(-2.80131,55.3077){1.20631}
\ECirc(-0.956784,56.5599){1.15038}
\ECirc(1.66773,57.4366){1.3407}
\ECirc(0.104403,55.0303){0.636102}
\ECirc(-2.24486,53.7507){3.23621}
\ECirc(10.9441,-25.61){3.53552}
\ECirc(43.3355,-12.0371){3.04219}
\ECirc(14.4009,7.42381){3.54345}
\ECirc(-17.1823,6.76105){3.5354}
\ECirc(-5.63118,-3.96617){0.83625}
\ECirc(4.99614,33.6483){3.51422}
\ECirc(32.1034,-21.7388){1.96449}
\ECirc(16.0907,-35.9964){3.54025}
\ECirc(13.8382,-49.2686){3.53515}
\ECirc(43.7573,4.76817){3.51376}
\ECirc(42.0929,8.93924){3.16513}
\ECirc(-28.5539,48.257){1.4251}
\ECirc(-28.2233,47.796){1.40043}
\ECirc(4.77873,-1.03285){3.56551}
\ECirc(-9.98232,26.1802){2.90198}
\ECirc(-11.7032,24.3886){1.35818}
\ECirc(-14.4721,30.032){1.11921}
\ECirc(-19.1255,23.3553){3.45991}
\ECirc(-8.81924,66.4419){3.17129}
\ECirc(7.14779,-58.911){3.53534}
\ECirc(-8.63908,5.53155){1.99856}
\ECirc(1.9079,5.10868){3.55139}
\ECirc(-39.8839,-8.0904){3.23295}
\ECirc(-46.927,-11.0034){1.36945}
\ECirc(-29.4085,-10.5191){1.23101}
\ECirc(28.2411,11.8521){3.53125}
\ECirc(55.2671,41.7561){3.53552}
\ECirc(59.2659,26.6513){3.39478}
\ECirc(52.9227,17.5171){3.42869}
\ECirc(-7.72042,47.8258){3.21068}
\ECirc(-9.91547,43.8056){2.13927}
\ECirc(-10.1866,43.8569){1.66726}
\ECirc(23.7288,-11.0834){3.53485}
\ECirc(-39.0412,1.0324){1.91095}
\ECirc(1.79004,22.3335){3.53387}
\ECirc(2.31946,-15.1761){3.53551}
\ECirc(7.71545,-19.3811){2.49156}
\ECirc(8.08685,-9.81295){3.53154}
\ECirc(45.6778,-21.7232){2.35971}
\ECirc(55.4194,-11.2772){1.31774}
\ECirc(57.1858,-11.8353){0.919441}
\ECirc(55.1587,-11.8689){1.17776}
\ECirc(-15.2223,-13.9205){3.53409}
\ECirc(-26.0276,51.9939){1.4979}
\ECirc(-22.0782,51.9012){2.95373}
\ECirc(-21.972,53.2624){3.52956}
\ECirc(-4.53487,-61.0104){3.44852}
\ECirc(0.631583,-62.3912){2.86936}
\ECirc(3.29969,-59.2029){2.36037}
\ECirc(2.05974,-56.6157){1.22302}
\ECirc(-47.4078,-19.5946){1.23273}
\ECirc(-23.1943,32.1586){2.43273}
\ECirc(24.8653,45.4144){3.53553}
\ECirc(-11.4981,-21.7873){2.47206}
\ECirc(-44.1077,-14.3974){3.51727}
\ECirc(-39.2615,-15.5388){3.52908}
\ECirc(10.9596,-25.1068){3.53553}
\ECirc(-39.5358,21.0139){3.52853}
\ECirc(-27.2161,34.6358){0.786281}
\ECirc(-34.9394,29.7809){0.830048}
\ECirc(11.3717,24.1699){2.78296}
\ECirc(17.025,20.5137){2.59313}
\ECirc(16.7015,20.7118){2.32913}
\ECirc(-1.36089,-18.4219){3.53509}
\ECirc(-1.02844,25.0811){2.02619}
\ECirc(-8.57488,29.6152){1.60411}
\ECirc(-4.47884,26.5311){1.7213}
\ECirc(-42.9676,-13.4838){2.61156}
\ECirc(-41.0585,-7.5599){3.53545}
\ECirc(-43.3302,-9.58922){3.14666}
\ECirc(-42.6065,-5.33424){2.19295}
\ECirc(-36.7692,-5.08014){0.831845}
\ECirc(-40.5125,-3.66843){0.365575}
\ECirc(0.131327,-3.1581){1.95152}
\ECirc(-1.00549,9.69309){1.43577}
\ECirc(-1.3873,8.97804){0.756393}
\ECirc(-2.18157,11.9199){1.0782}
\ECirc(-4.16078,17.4246){2.32952}
\ECirc(67.567,-16.6789){3.45542}
\ECirc(4.53564,29.7613){2.91917}
\ECirc(-12.6451,0.295088){3.53598}
\ECirc(-4.62445,-3.91878){3.51018}
\ECirc(-30.2272,46.0515){3.03342}
\ECirc(-27.4094,38.7179){3.53267}
\ECirc(-1.80254,-57.4625){3.53538}
\ECirc(7.48423,-4.31471){3.53517}
\ECirc(-26.9003,46.7641){3.53525}
\ECirc(-25.9801,48.875){2.38637}
\ECirc(-24.2139,45.0628){2.59632}
\ECirc(-29.7294,43.0838){2.78929}
\ECirc(13.6313,-4.89975){3.53499}
\ECirc(4.42483,-5.31474){0.951656}
\ECirc(7.11955,0.00137241){3.09307}
\ECirc(-7.07234,30.7699){3.50717}
\ECirc(-10.02,28.8686){2.11737}
\ECirc(-3.91327,34.0442){2.87907}
\ECirc(-14.073,30.2439){3.43804}
\ECirc(-4.57128,35.916){1.92361}
\ECirc(-6.70986,19.9738){3.53127}
\ECirc(-10.3504,17.8761){2.03899}
\ECirc(-39.3177,16.2479){3.50893}
\ECirc(-4.18638,15.9536){2.10346}
\ECirc(31.7722,47.1977){2.39784}
\ECirc(20.7968,39.9201){1.42831}
\ECirc(20.9503,40.293){1.37408}
\ECirc(20.2813,49.4743){2.22498}
\ECirc(23.808,-32.9417){2.53075}
\ECirc(-14.9371,-21.5887){2.2037}
\ECirc(-30.1291,-9.87727){2.44224}
\ECirc(-16.7743,-16.781){2.87622}
\ECirc(-23.3847,58.142){3.53548}
\ECirc(-17.4931,-25.401){3.53534}
\ECirc(40.8184,30.9194){1.17536}
\ECirc(38.0196,34.1628){3.44724}
\ECirc(8.4308,-32.4533){1.68708}
\ECirc(10.5556,-20.3257){1.3173}
\ECirc(7.10335,-18.5267){2.67043}
\ECirc(7.50291,-17.9631){2.78823}
\ECirc(7.53561,-13.7876){3.53535}
\ECirc(59.5472,-6.33681){1.69033}
\ECirc(56.056,-0.473242){3.53508}
\ECirc(16.6567,-17.3519){1.50499}
\ECirc(-30.314,-8.72116){3.53546}
\ECirc(-27.6673,-22.5491){1.61422}
\ECirc(-12.6575,26.5807){2.72743}
\ECirc(-13.0447,24.1886){3.42023}
\ECirc(-50.9841,47.4045){0.874112}
\ECirc(-47.2263,46.8673){1.83781}
\ECirc(-34.5577,30.3912){3.53544}
\ECirc(0.560325,-3.85109){1.59326}
\ECirc(2.50071,0.4373){2.59231}
\ECirc(7.33729,1.57158){2.52988}
\ECirc(48.1384,16.8952){3.53462}
\ECirc(-52.9789,-19.4345){3.53533}
\ECirc(-30.4107,5.07051){3.12269}
\ECirc(-36.2371,5.32447){3.22435}
\ECirc(-40.3403,0.617112){0.788695}
\ECirc(-39.3121,-0.429528){2.18524}
\ECirc(-7.31002,7.02181){0.822066}
\ECirc(-9.20261,0.760931){0.795081}
\ECirc(-10.3482,2.00481){1.94845}
\ECirc(7.38539,7.48526){3.31644}
\ECirc(5.58687,38.5808){3.53541}
\ECirc(6.02219,37.5327){1.78058}
\ECirc(6.12793,36.4569){0.781539}
\ECirc(5.90733,37.898){1.35912}
\ECirc(-17.1701,-38.829){1.6162}
\ECirc(-17.7565,-37.0014){2.09979}
\ECirc(-23.6756,-34.3757){2.38734}
\ECirc(18.4965,23.2019){1.96766}
\ECirc(-4.47779,-42.2551){3.48282}
\ECirc(-6.39647,-45.5663){1.49822}
\ECirc(-52.7758,23.1306){3.53496}
\ECirc(-23.8123,-27.0551){1.66865}
\ECirc(-28.1094,-23.8209){2.37453}
\ECirc(-33.0216,-11.9398){3.23233}
\ECirc(45.3227,31.8441){0.456196}
\ECirc(21.3569,3.36657){3.35023}
\ECirc(25.3635,7.39585){1.66457}
\ECirc(23.7286,2.42662){1.27421}
\ECirc(23.7513,0.409238){3.53502}
\ECirc(27.3238,6.00153){0.616912}
\ECirc(29.705,2.3831){1.12431}
\ECirc(25.8462,4.72436){3.34375}
\ECirc(-5.37518,15.4348){3.53552}
\ECirc(36.4593,4.5382){0.412953}
\ECirc(39.2882,3.05999){2.74666}
\ECirc(36.3481,3.78794){1.26597}
\ECirc(41.618,6.08093){3.53355}
\ECirc(42.51,5.76634){3.24637}
\ECirc(42.3152,8.07601){3.50599}
\ECirc(-3.04211,-26.3319){3.53446}
\ECirc(1.72784,-30.363){1.06369}
\ECirc(3.60037,-31.2472){1.9684}
\ECirc(-3.23255,-26.7291){0.757983}
\ECirc(-4.1082,-25.8753){1.34261}
\ECirc(4.60582,-21.2914){1.15485}
\ECirc(44.6522,27.0698){0.975145}
\ECirc(41.0343,25.2242){0.633458}
\ECirc(40.692,32.0236){3.11787}
\ECirc(39.9631,40.8612){1.50451}
\ECirc(41.3678,35.7549){2.92781}
\ECirc(-26.0901,70.3643){3.53553}
\ECirc(31.1288,-47.7116){3.45354}
\ECirc(27.0013,-39.603){2.99719}
\ECirc(5.81591,3.09002){3.485}
\ECirc(-2.34807,-5.48137){2.28575}
\ECirc(-7.27721,-26.5933){3.53553}
\ECirc(-7.58419,-39.6094){1.54143}
\ECirc(-6.37331,-40.7183){1.00245}
\ECirc(-5.27814,-40.1467){1.62589}
\ECirc(29.1402,46.4086){2.79954}
\ECirc(26.946,51.7212){3.3831}
\ECirc(25.9056,55.5702){3.52246}
\ECirc(29.87,-32.1513){3.14067}
\ECirc(17.7425,-39.4906){1.82381}
\ECirc(15.7787,-42.2523){2.55441}
\ECirc(18.1914,-40.0413){3.52985}
\ECirc(28.2905,-26.3143){3.53518}
\ECirc(25.9902,-24.0379){2.88594}
\ECirc(29.5462,-30.0541){1.32624}
\ECirc(32.4299,-22.3766){0.663957}
\ECirc(-19.5662,-4.76511){0.737931}
\ECirc(-18.3033,-13.1618){2.15674}
\ECirc(-19.182,-16.7088){0.63227}
\ECirc(-20.1607,-15.2825){0.919116}
\ECirc(-12.618,-11.4747){3.27611}
\ECirc(5.6073,-22.0118){3.21891}
\ECirc(3.84968,-26.4945){3.35987}
\ECirc(4.73779,-27.8942){2.31338}
\ECirc(6.60212,-26.4608){2.26994}
\ECirc(-21.3052,-14.4712){3.52162}
\ECirc(32.4173,28.3206){3.50416}
\ECirc(36.4026,24.0379){1.46418}
\ECirc(33.5818,27.9031){3.5179}
\ECirc(30.9046,30.4827){3.53511}
\ECirc(8.91341,-13.7694){3.53552}
\ECirc(-36.6872,49.3779){1.80053}
\ECirc(-25.2134,46.9807){3.53544}
\ECirc(-32.8572,-34.1511){1.39717}
\ECirc(-34.2281,-42.0413){2.18349}
\ECirc(18.0341,-22.8573){1.78788}
\ECirc(-44.2576,-3.58818){0.62829}
\ECirc(21.8849,-9.6651){3.47896}
\ECirc(44.4247,-0.2494){3.53545}
\ECirc(38.9283,2.92528){1.38585}
\ECirc(2.17008,11.4826){3.53538}
\ECirc(1.02652,15.0999){3.53541}
\ECirc(46.1446,22.5204){0.775133}
\ECirc(-35.0683,-32.7119){1.5014}
\ECirc(-10.3867,32.4688){1.66999}
\ECirc(-60.2221,18.8476){3.53553}
\ECirc(-23.0744,2.41604){3.54048}
\ECirc(-20.997,59.6748){2.42088}
\ECirc(-20.5526,51.3656){3.53519}
\ECirc(14.7954,0.120112){1.93975}
\ECirc(38.2995,-1.386){3.49942}
\ECirc(-25.8261,2.15758){1.45842}
\ECirc(-27.5543,8.84534){2.73377}
\ECirc(-48.7304,-22.1226){3.53408}
\ECirc(29.8044,-11.6089){1.19285}
\ECirc(18.4802,-18.5176){1.43164}
\ECirc(14.7071,-20.075){1.49185}
\ECirc(14.2523,-21.3343){2.78631}
\ECirc(18.4526,-22.9801){0.512325}
\ECirc(12.3886,-34.5157){3.53551}
\ECirc(-3.55787,44.7837){2.4482}
\ECirc(-38.2161,-36.9227){3.53552}
\ECirc(-32.4647,-35.0552){3.37294}
\ECirc(-53.7409,42.6631){2.41352}
\ECirc(-1.42688,-48.0776){2.28493}
\ECirc(-0.710663,-43.8423){3.33939}
\ECirc(3.98738,-42.2063){2.03894}
\ECirc(-28.2215,33.3163){3.52392}
\ECirc(-34.6875,35.3593){3.53271}
\ECirc(45.1257,28.3776){3.52721}
\ECirc(49.3126,22.2824){2.02106}
\ECirc(40.6992,25.7927){2.03991}
\ECirc(47.3802,25.4398){3.53525}
\ECirc(17.7511,-8.18143){3.53548}
\ECirc(8.91952,-21.2502){3.53487}
\ECirc(18.8497,-52.4788){3.53553}
\ECirc(-14.6899,-47.4236){1.81764}
\ECirc(-3.32457,-9.80466){2.47639}
\ECirc(-37.9382,-2.22091){3.53553}
\ECirc(9.83588,-15.1339){3.23285}
\ECirc(6.22588,-12.0386){2.07504}
\ECirc(9.01143,-16.6506){0.941182}
\ECirc(10.139,-21.368){1.42288}
\ECirc(69.6497,15.9235){3.53534}
\ECirc(46.7345,-46.463){3.51114}
\ECirc(-19.7195,-23.7074){3.52514}
\ECirc(8.01729,19.9095){3.47692}
\ECirc(-32.9382,30.549){3.53553}
\ECirc(-37.0096,41.5579){3.2908}
\ECirc(65.9264,-19.7076){2.66339}
\ECirc(4.43778,-14.7589){3.52559}
\ECirc(3.93381,-8.84956){2.77827}
\ECirc(3.30715,-9.31675){2.8426}
\ECirc(-0.0182838,-7.53014){3.34588}
\ECirc(-2.88906,-4.74483){3.47355}
\ECirc(10.3621,-11.8959){1.73521}
\ECirc(5.96474,-13.2953){3.51587}
\ECirc(-7.31599,-23.4682){2.07099}
\ECirc(-4.78929,-27.9328){3.53417}
\ECirc(-2.17558,-28.5436){1.59614}
\ECirc(-1.18404,-24.4384){2.16456}
\ECirc(-4.93367,-25.4393){1.05696}
\ECirc(-5.97725,-26.597){1.47383}
\ECirc(-2.71402,-23.3358){3.50227}
\ECirc(30.1898,58.7078){1.96971}
\ECirc(-18.2234,20.6068){3.51939}
\ECirc(-58.2129,15.1006){3.50483}
\ECirc(-60.8637,23.0345){1.76574}
\ECirc(-49.8392,13.4296){0.801153}
\ECirc(-49.3501,13.0083){1.14625}
\ECirc(-55.8828,22.061){1.76687}
\ECirc(-10.9194,-35.3664){2.1465}
\ECirc(-3.74437,-53.008){3.52471}
\ECirc(39.5554,-41.7769){3.22394}
\ECirc(29.7706,68.5157){0.829607}
\ECirc(9.21011,9.30936){2.70167}
\ECirc(17.5597,32.9792){0.442074}
\ECirc(19.9195,27.8207){2.93949}
\ECirc(27.539,15.9807){2.76943}
\ECirc(-17.1951,22.8054){3.14298}
\ECirc(-19.945,24.8041){3.37189}
\ECirc(-19.6025,24.4827){3.3377}
\ECirc(-16.3362,20.3961){2.09948}
\ECirc(-16.3316,19.154){2.57207}
\ECirc(27.7129,40.2278){1.58673}
\ECirc(-49.9919,23.5421){2.62699}
\ECirc(27.1588,-21.3681){3.5352}
\ECirc(30.4421,-27.08){3.48242}
\ECirc(21.2792,3.66968){2.17665}
\ECirc(12.288,2.84155){2.58347}
\ECirc(13.4352,11.8546){1.79067}
\ECirc(41.0384,-23.6903){3.10815}
\ECirc(45.8386,-21.6041){1.74078}
\ECirc(42.3295,-26.8012){3.19851}
\ECirc(42.9132,-22.6735){3.53546}
\ECirc(42.7243,-21.1663){3.53387}
\ECirc(65.2647,18.0984){3.51707}
\ECirc(-12.6847,-15.1155){1.86895}
\ECirc(-4.02661,-10.8376){2.44728}
\ECirc(-6.54929,-14.4742){2.47292}
\ECirc(-16.0941,-12.1361){1.88698}
\ECirc(-61.5388,-18.9674){3.53553}
\ECirc(11.0253,-32.833){2.60654}
\ECirc(11.6879,-31.4525){3.08689}
\ECirc(11.978,-29.7393){3.49874}
\ECirc(3.02794,-29.132){1.20994}
\ECirc(58.5916,28.722){3.44787}
\ECirc(28.7437,9.5381){3.35057}
\ECirc(32.6814,16.9044){1.23734}
\ECirc(31.402,17.8001){1.63089}
\ECirc(-65.2455,16.2693){3.53553}
\ECirc(-13.5499,63.1824){1.80441}
\ECirc(-30.9326,-32.808){1.45888}
\ECirc(20.3528,33.1987){2.01298}
\ECirc(-24.4677,73.8569){2.79035}
\ECirc(-51.0914,-2.07077){1.6084}
\ECirc(-32.0124,-14.1372){3.53546}
\ECirc(-25.229,-6.70943){3.53553}
\ECirc(-30.2383,-14.0131){1.06385}


==> figs/pp-1.tex <==
\ECirc(-0.149183,1.59019){0.61653}
\ECirc(4.34488,1.90703){0.627169}
\ECirc(0.903395,-3.02356){0.410113}
\ECirc(3.12828,-0.16264){0.702091}
\ECirc(3.68788,2.19048){0.982788}
\ECirc(1.9798,-0.814876){0.645915}
\ECirc(1.98294,2.13183){0.706242}
\ECirc(4.67148,2.24996){0.44752}
\ECirc(4.3804,1.20164){0.226586}
\ECirc(3.97757,1.3208){0.236335}
\ECirc(1.25273,1.37447){1.15783}
\ECirc(0.81926,1.42296){0.737332}
\ECirc(4.4995,1.37173){0.680775}
\ECirc(-0.0909131,-0.548962){1.12533}
\ECirc(1.99188,0.15369){0.505679}
\ECirc(4.04706,-2.34487){0.537866}
\ECirc(2.29886,3.26773){0.505351}
\ECirc(5.02416,0.531592){0.379255}
\ECirc(3.75185,0.391654){2.07941}
\ECirc(4.48086,0.723449){0.519506}
\ECirc(3.32225,0.578816){0.519506}
\ECirc(3.20813,0.480713){0.799727}
\ECirc(1.41842,2.02773){0.694761}
\ECirc(0.0528013,-0.0812315){0.180177}
\ECirc(-0.364374,-1.83754){0.178151}


==> figs/pp-3.tex <==
\ECirc(-1.14394,2.31113){1.67393}
\ECirc(4.49228,2.81892){1.88151}
\ECirc(1.12219,-4.67172){1.17906}
\ECirc(3.20758,0.061547){2.10627}
\ECirc(3.58275,3.88045){1.12897}
\ECirc(1.33595,-1.31269){1.93774}
\ECirc(2.08161,2.12561){2.11873}
\ECirc(5.78894,1.178){1.34256}
\ECirc(4.82735,-0.730991){0.270736}
\ECirc(3.99576,-0.564093){0.709006}
\ECirc(0.38073,2.41738){1.55594}
\ECirc(-0.0401794,3.01722){0.899815}
\ECirc(4.99812,1.16258){2.04233}
\ECirc(-1.74509,-1.25963){1.12533}
\ECirc(1.02407,-0.855093){1.51704}
\ECirc(5.25307,-0.887279){0.688187}
\ECirc(3.93154,2.25838){0.595834}
\ECirc(6.65335,-0.526652){0.504065}
\ECirc(3.61122,1.07991){2.07941}
\ECirc(6.13413,1.82498){0.519506}
\ECirc(4.9834,1.68019){0.519506}
\ECirc(3.87795,0.268737){1.98613}
\ECirc(1.17949,2.31299){2.08428}
\ECirc(0.294264,1.89885){0.180177}
\ECirc(-0.125481,0.145284){0.178151}


==> figs/pp-5.tex <==
\ECirc(-2.1387,3.03206){2.78988}
\ECirc(4.63968,3.73081){3.13585}
\ECirc(1.34099,-6.31988){1.96509}
\ECirc(3.28688,0.285734){3.51045}
\ECirc(3.47761,5.57041){1.88162}
\ECirc(0.692111,-1.81051){3.22957}
\ECirc(2.18028,2.1194){3.53121}
\ECirc(6.90639,0.106035){2.2376}
\ECirc(5.2743,-2.66363){0.451227}
\ECirc(4.01395,-2.44899){1.18168}
\ECirc(-0.491267,3.46029){2.59323}
\ECirc(-0.899619,4.61147){1.49969}
\ECirc(5.49673,0.95343){3.40388}
\ECirc(-3.39926,-1.97029){1.53975}
\ECirc(0.0562504,-1.86388){2.5284}
\ECirc(6.45907,0.570312){1.14698}
\ECirc(5.56422,1.24903){0.993057}
\ECirc(8.28254,-1.5849){0.840109}
\ECirc(3.47059,1.76818){3.31027}
\ECirc(7.78741,2.92652){0.519506}
\ECirc(6.64455,2.78156){0.519506}
\ECirc(4.54778,0.0567609){3.31021}
\ECirc(0.940568,2.59826){3.4738}
\ECirc(0.535726,3.87893){0.256014}
\ECirc(0.113412,2.12811){0.18834}

